Covert Channel-Based Transmitter Authentication in Controller Area Networks

In recent years, the security of automotive Cyber-Physical Systems (CPSs) is facing urgent threats due to the widespread use of legacy in-vehicle communication systems. As a representative legacy bus system, the Controller Area Network (CAN) hosts Electronic Control Units (ECUs) that are crucial vehicle functioning. In this scenario, malicious actors can exploit CAN vulnerabilities, such as the lack of built-in authentication and encryption schemes, to launch CAN bus attacks with life-threatening consequences (e.g., disabling brakes). In this paper, we present TACAN (Transmitter Authentication in CAN), which provides secure authentication of ECUs on the legacy CAN bus by exploiting the covert channels, without introducing CAN protocol modifications or traffic overheads. TACAN turns upside-down the originally malicious concept of covert channels and exploits it to build an effective defensive technique that facilitates transmitter authentication via a centralized, trusted Monitor Node. TACAN consists of three different covert channels for ECU authentication: 1) the Inter-Arrival Time (IAT)-based; 2) the Least Significant Bit (LSB)-based; and 3) a hybrid covert channel, exploiting the combination of the first two. In order to validate TACAN, we implement the covert channels on the University of Washington (UW) EcoCAR (Chevrolet Camaro 2016) testbed. We further evaluate the bit error, throughput, and detection performance of TACAN through extensive experiments using the EcoCAR testbed and a publicly available dataset collected from Toyota Camry 2010. We demonstrate the feasibility of TACAN and the effectiveness of detecting CAN bus attacks, highlighting no traffic overheads and attesting the regular functionality of ECUs.

==> Sections/acknoledgments.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi

The authors would like to thank...

==> Sections/appendices.tex <==
\newpage

\balance
\appendices
% \section{CAN Frame}
% \label{appendix:CAN_frame}
% As illustrated in Figure~\ref{fig:can_frame_structure}, each CAN frame or message has a set of predefined fields, including the Start of Frame (SOF) field, the Arbitration field (including a 11-bit message ID for the base frame format or a 29-bit message ID for the extended frame format), the Control field, the Data field (8-64 bits), the CRC field, the ACK field, and the End of Frame (EOF) field.

% \begin{figure}[ht!]
% \centering
% \includegraphics[width=1\columnwidth]{./Figures/can_frame_structure}
% \caption{Illustration of CAN frame structure.}
% \label{fig:can_frame_structure}
% \vspace{-0.3cm}
% \end{figure}

\section{Impact on CAN Bus Schedulability}
\label{appendix:schedulability}
In order to understand the impact of the timing parameter $\delta$ introduced by the IAT-based covert channel in TACAN on CAN bus schedulability, we apply the schedulability analysis in \cite{davis2007controller}.
For the ease of discussion, we provide a summary of definitions as below. 
%The same notations in \cite{davis2007controller} are used for consistency.
\begin{itemize}
    \item $k$: Message priority, which is used interchangeably with the message ID.
    \item $C_k$: Transmission time, defined as the longest time that the message can take to be transmitted.
    \item $J_k$: Queuing jitter, defined as the longest time between the initiating event and the message being queued, ready to be transmitted on the bus.
    \item $w_k$: Queuing delay, defined as the longest time that the message can remain in the CAN controller slot or device driver queue, before commencing successful transmission on the bus.
    \item $T_k$: Message period, defined as the minimum inter-arrival time of the event that triggers queueing of the message. 
    Such events may occur strictly periodically with a period of $T_k$ or sporadically with a minimum separation of $T_k$. 
    \item $R_k$: Worst-case response time of message $k$, defined as the longest time from the initiating event occurring to the message being received by the nodes that require it.
    \item $D_k$: Hard deadline, defined as the maximum permitted time from occurrence of the initiating event to the end of successful transmission of the message. 
\end{itemize}
A message is \textit{schedulable} if and only if its worst-case response time is no greater than its deadline ($R_k \leq D_k$). 
A CAN bus is schedulable if and only if all messages on the CAN bus are schedulable.

As per \cite{davis2007controller}, we have $C_k = (80 + 10 s_k)\tau_{bit}$ (including bit stuffing), where $s_k$ is the number of data bytes and $\tau_{bit}$ is the transmission time of a single bit. 
For a $8$-byte message on a $500$ kbps CAN bus, we have $\tau_{bit}=2~\mu$s and  $C_k=320$ $\mu$s.
While CAN nodes typically have separate clock sources, all the timing quantities (e.g., message jitters, bit times, message periods, and deadlines) that derived from node clocks will be converted to real-time. 

The message $k$'s worst-case response time $R_k$ is given by
\begin{equation*}
    R_k = J_k + w_k + C_k,
\end{equation*}
and the queuing delay $w_k$ consists of two elements:
\begin{itemize}
    \item \textit{Blocking} $B_k$, due to lower priority messages  being transmitted when message $k$ is queued, and
    \item \textit{Interference} due to higher priority messages which may win arbitration and be transmitted in preference to message $k$.
\end{itemize}
The blocking delay is given by $B_k = \max_{i \in lp(k)} (C_i)$, where $lp(k)$ is the set of messages with lower priority than $k$.

In order to analyze the worst-case response time, it is important to characterize the busy period, where all messages of priority $k$ or higher, queued strictly before the end of busy period, are transmitted during the busy period. 
The maximal busy period begins with a so-called critical instant where message $k$ is queued simultaneously with all higher priority messages and then each of these higher priority messages is subsequently queued again after the shortest possible time interval.

For simplicity, we assume that only one instance of message $k$ is transmitted during a priority level-$k$ busy period. 
In this case, the worst-case queuing delay is 
\begin{equation}\label{eq:worst_case_queuing_delay}
    w_k = B_k + \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k + J_i + \tau_{bit}}{T_i}  \right\rceil C_i.
\end{equation}
Since the right hand side is a monotonic non-decreasing function of $w_k$, Eq.~(\ref{eq:worst_case_queuing_delay}) can be solved using the following recurrence relation,
\begin{equation}\label{eq:worst_case_queuing_delay2}
    w_k^{n+1} = B_k + \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k^n + J_i + \tau_{bit}}{T_i} \right\rceil C_i.
\end{equation}
A suitable starting value is $w_k^0 = B_k$, and the recurrence relation iterates until, either $J_k + w_k^{n+1} + C_k > D_k$, i.e., the message is not schedulable, or $w_k^{n+1}=w_k^n$, in which case the worst-case response of message $k$ is given by $J_k + w_k^{n+1}+C_k$. 

In order to apply the above schedulability analysis to TACAN, we define $T'_k = T_k - \delta$. 
Since TACAN adds at most $\delta$ to each ITT, which can be considered as part of the queuing jitter, we have $J'_k=J_k + \delta$. 
Assume that $\delta = 0.01 T_k$ and all messages employ the IAT-based covert channel. 
By substituting $T'_k=0.99 T_k$ and $J'_m=J_m + 0.01 T_k$ into Eq.~(\ref{eq:worst_case_queuing_delay2}), we have
\begin{align}
    w_k^{' n+1} &= B_k + \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k^{' n} + (J_i + 0.02 T_i) + \tau_{bit}}{0.98 T_i} \right\rceil C_i \nonumber\\
    &\approx B'_k  + 
    \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k^{' n} + J_k + \tau_{bit}}{T_i} \right\rceil C'_i, \label{eq:updated_worst_case_queuing_delay}
\end{align}
where 
\begin{equation}\label{eq:appendix:blocking_delay}
    B_k' = B_k + \sum_{\forall i \in hp(k)} \left(\frac{0.01}{0.99} C_i \right), 
\end{equation}
and 
\begin{equation}\label{eq:appendix:msg_tx_time}
    C'_i = \frac{1}{0.99} C_i = 1.01 C_i.
\end{equation}
Therefore, the impact of $\delta$ on the worst-case response time is threefold: 1) increasing the queuing jitter by a fixed amount of time, 2) increasing the blocking delay by a bounded amount of time, and 3) increasing the equivalent message transmission time of higher priority messages by a certain percentage.

As an example, let us consider a 10-ms message and set $\delta=0.01T=0.1$ ms. 
Then the increase in the queuing jitter is $100~\mu$s. 
Assuming 45 higher priority messages (half of the messages on the EcoCAR \cite{ecocar}) with 8-byte data on a 500 kbps bus ($C_i=320~\mu$s), the increase in the blocking delay is $145~\mu$s (Eq.~(\ref{eq:appendix:blocking_delay})). 
In addition, the equivalent increase in the message transmission time of each higher priority message is $1\%$, which is equal to $3.2~\mu$s (Eq.~(\ref{eq:appendix:msg_tx_time})). 
By solving Eq.~(\ref{eq:updated_worst_case_queuing_delay}), we can compute the corresponding worst-case response time of message $k$ with TACAN. 
%The above discussion suggests that schedulability tests will need to be performed during TACAN configurations to ensure the schedulability of the system.
Hence, to achieve effective use of covert channels, the TACAN parameter $\delta$ needs to be experimentally obtained and fine tuned prior to deployment to ensure the schedulability of the CAN bus.



==> Sections/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> Sections/discussion.tex <==
\section{Discussion}
\shaun{Should we keep this section or not?}

\subsection{Impact of Missing Messages}

\subsection{Use of Error Correction Code}
When the probability of bit errors is reasonably small, one may also consider Error Correction Coding (ECC) techniques that are widely used in communications \cite{goldsmith2005wireless} to detect and recover occasional bit errors. 
\rev{Nevertheless, the use of ECC techniques will unavoidably complicates the design of covert channels and introduces overheads.
In addition, since the probability of consecutive corrupted authentication frames is small, it is acceptable to not recover the bit errors in a particular frame.}

\subsection{Detection Delays}

\subsection{A Communication Channel Perspective}
How to improve channel throughput? 

Tradeoff between throughput and length 

\begin{itemize}
    \item Capacity
    \item Non-return-to-zero (NRZ)
    \item Error correction code
    \item Multiple levels
    \item CRC
\end{itemize}

==> Sections/security_analysis.tex <==
\section{Security Discussion \shaun{(To be updated)}}
\label{sec:security_analysis}
%In this section, we provide a security discussion of TACAN.
Compared to the existing message authentication schemes \cite{herrewege2011canauth,hazem2012lcap,kurachi2014cacan,radu2016leia} that attempt to verify the authenticity of each message, TACAN extracts and verifies authentication message embedded in the timing or LSBs of normal messages to authenticate the transmitting ECU and also serves the purpose of intrusion detection.
%While TACAN cannot detect spoofed messages (since it does not examine the message content), 
Hence, TACAN can detect attacks that interrupt the transmission of normal CAN messages (e.g., suspension, injection, and DoS attacks), as well as attacks in which attackers fail to generate valid authentication messages (e.g., forgery, replay, and masquerade attacks). 
The above security properties provided by TACAN are independent of the CAN protocol and the contents of CAN messages.
%The main advantage of TACAN is that it does not require protocol modifications or introduce traffic overheads (i.e., no extra bits or messages).
%Moreover, since ECUs are resource-constrained and authentication message generation can be computationally expensive, TACAN can significantly reduce the computational burden on ECUs by requiring them to transmit authentication messages much less frequently than per-message authentication schemes.
%In the rest of this section, we will discuss how TACAN is able to detect the aforementioned attacks in more detail.
%\revv{In the rest of this section, we will discuss the security features of TACAN and how it detects forgery, replay, and masquerade attacks in more detail.}

%In particular, we discuss how TACAN is able to detect forgery, replay, and masquerade attacks.

\vspace{0.1cm}
\noindent \textbf{Security Features.}
We summarize a list of features provided by TACAN as follows: 1) TACAN securely stores both master and session keys in the ECU's TPM to prevent being compromised by the adversary, 2) TACAN employs monotonic counters for generating session keys and authentication messages for each ECU, and 3) TACAN requires each ECU to continuously transmit unique authentication messages to enable real-time transmitter authentication.

Note that due to the third feature, if the attacker compromises an in-vehicle ECU but does not attempt to deceive TACAN (i.e., stop generating authentication messages), it will interrupt the continuous transmission of authentication messages and thus will be detected immediately.
In addition, since basic attacks like suspension, injection, and DoS attacks can be easily detected, we focus on more sophisticated attacks in the rest of this section that actively attempt to evade TACAN, including the forgery attack, the replay attack, and the masquerade attack.

\vspace{0.1cm}
\noindent \textbf{Detecting Forgery Attacks.}
In the forgery attack, the adversary has already compromised an in-vehicle ECU that is protected by TACAN and attempts to generate valid authentication messages that can be verified by the MN in order to evade the detection of TACAN. 
Since our adversary model (Section~\ref{sec:adversary_model}) assumes that the attacker has no access to the TPM of the compromised ECU, the attacker has to forge a valid digest for each local counter value without the session key.
With a condensed digest of $M$ bits, the probability of a successful forgery is $1/2^M$.
For example, when $M=8$, this probability is $1/2^8 \approx 0.4\%$.
Repeated forgeries will be prevented due to the use of monotonic counters. 

\vspace{0.1cm}
\noindent \textbf{Detecting Replay Attacks.}
A replay attacker has infiltrated the CAN bus and attempts to replay previously transmitted authentication messages of the targeted ECU with the hope of passing the verification process at the MN.
It is easy to see that such attempts will be detected by TACAN due to the use of monotonic counters. 

% \vspace{0.1cm}
% \noindent \textbf{Detecting Compromised ECUs.}
% Our adversary model (Section~\ref{sec:adversary_model}) assumes that the attacker has no access to both the master and session keys stored in the TPM of the compromised ECU.
% In order to deceive TACAN, the attacker has to forge a valid digest for each local counter value without the session key.
% With a condensed digest of $M$ bits, the probability of a successful forgery is $1/2^M$.
% For example, when $M=8$, this probability is $1/2^8 \approx 0.4\%$.
% Repeated forgeries and replay attacks will not work because the local counter is incremented monotonically. 
% Therefore, a compromised ECU will be detected by TACAN with very high probability.

% \vspace{0.1cm}
% \noindent \textbf{Detecting Suspension Attacks.}
% Since a suspension attack requires a compromised in-vehicle ECU, this attack will be readily detected by TACAN, according to our previous discussion.
% Moreover, suspending a CAN message that carries authentication messages between the ECU and the MN will also interrupt the underlying covert channel, which can be detected by the MN. 

% \vspace{0.1cm}
% \noindent \textbf{Detecting Fabrication Attacks.}
% If the fabrication attack requires compromising an in-vehicle ECU, it will be detected by TACAN; otherwise, it needs to be launched from an external device.
% There are two cases of message fabrication.
% In the first case, non-existent message IDs are used (e.g., using 0x00 for launching the DoS attack). 
% Such attacks will not be detected directly by TACAN. 
% In the second case, existing message IDs are used.
% The attack will be detected by TACAN, if the targeted message is used to deploy the covert channel. 
% In either case, if the attacker introduces abnormal CAN traffic that interrupts the deployed covert channels, TACAN will raise an alarm. 
% Nevertheless, existing IDSs such as \cite{hoppe2008security,miller2013adventure} can always be deployed in conjunction with TACAN to enhance the CAN bus security.

\vspace{0.1cm}
\noindent \textbf{Detecting Masquerade Attacks.}
As mentioned in Section~\ref{sec:adversary_model}, a masquerade attack (including the more sophisticated cloaking attack \cite{sagong2018cloaking}) requires in-vehicle ECUs to be weakly and/or fully compromised.
As a result, TACAN will force the attacker to perform a forgery or replay attack, not only for the compromised ECU itself, but also for the ECU the attacker attempts to masquerade as. 
Therefore, a masquerade attack will be detected by TACAN. 
% , which can be detected by the TACAN before the onset of the attack.
% In addition, since a masquerading attacker has no access to the keys stored in the TPM of the targeted ECU, it will not be able to forge valid authentication messages that can pass the verification process at the MN. 

% \shaun{As mentioned in Section~\ref{sec:adversary_model}, a stealthy masquerade attack would require in-vehicle ECUs to be weakly and/or fully compromised, which can be detected by the MN before the onset of the attack.
% In general, when a compromised ECU or an external device attempts to masquerade as another ECU (by simply faking the message ID), the authentication message transmission of the targeted ECU may be interrupted, thus causing the MN to raise an alarm.
% Moreover, since the adversary has no access to the keys stored in the TPM of the targeted ECU, it will not be able to generate valid authentication sequences anyway. }

%In order to launch stealthy masquerade attacks, the attacker will need to compromise two ECUs -- one is weakly compromised and the other one is fully compromised \cite{lin2012cyber,cho2016finger}. 
%During the attack, the attacker suspends the weakly compromised ECU A from transmitting certain messages and uses the fully compromised ECU B to inject messages claiming to originate from ECU A. 
%As we can see, since the attacker has no access to the ECU A's private key, it will not be able to generate valid authentication messages for ECU A, and blind forgery can hardly succeed as discussed in the previous section.
%The premise that two ECUs need to be compromised already allows the MN to identify compromised ECUs and prevent masquerade attacks from happening.

\vspace{0.1cm}
% \noindent \textbf{Robustness Against Replay Attacks.}
% While the attacker is able to observe the current and all previous authentication messages transmitted by the targeted ECU, it is computationally unfeasible to launch replay attacks due to the built-in local counter in authentication messages. 
% Whenever the local counter overflows, the global counter will be incremented by one and a new session key will be generated. 
% Since each session key should be used only once for the lifetime of the vehicle, the same local counter value will not be signed by the same session key twice, which makes replay attacks extremely difficult, if not impossible. 

%\vspace{0.1cm}
% \noindent \textbf{Robustness Against Other Attacks.}
% In practice, it is possible to launch other attacks such as the suspension, fabrication, and DoS attacks.
% \shaun{If an attack (e.g., suspension attack) requires an in-vehicle ECU to be compromised, it can be readily detected by TACAN.}
% \shaun{On the one hand, if TACAN is deployed for all messages and the attacker injects messages with existing IDs, the resulting authentication message for the spoofed CAN message will fail the verification process at the MN and an alarm will be triggered.
% On the other hand, message injection using non-existence IDs can be easily detected, even without TACAN.}
% In practice, existing IDSs such as \cite{hoppe2008security,miller2013adventure} can also be deployed in conjunction with TACAN to enhance the CAN bus security.


==> Sections/tacan_offset_based.tex <==
\subsection{Offset-Based Covert Channel}
\label{sec:offset_based}
The idea of the offset-based covert channel is very similar to the IAT-based covert channel (Figure~\ref{fig:timing_based_scheme}).
The main difference is that the former performs running average on IATs (including the added deviations) to smooth out the noise, while the later aims to accumulate the deviations to differentiate the modulated samples from noise. 
Our observations about clock offsets are as follows. 

\vspace{0.1cm}
\noindent \textbf{Observations.}
According to our timing model in Section~\ref{sec:system_model} and Eq.~(\ref{eq:arrival_timestamp}), we have $t_i=\sum_{j=1}^i \Delta t_j$, $a_0=\eta_0$, and $a_i=t_i/(1+S)+\eta_i$. 
Since the receiver only knows the nominal period ($T$) of the targeted message, it computes the observed clock offset as the difference between the expected elapsed time (up to message $i$) at the transmitter and the actual elapsed time at the receiver, i.e.,
\begin{equation}
    \hat{O}_i = iT - (a_i - a_0) = iT - \frac{1}{1+S} \sum_{j=1}^i \Delta t_j + \eta_0 - \eta_i. \nonumber
\end{equation}
As we can see, if the transmitter adds $\delta$ to $L$ consecutive ITTs ($\Delta t_j = T+\delta$ for $j=1,...,L$), the deviations will accumulate and lead to a decrease of $\delta L/(1+S)$ in $\hat{O}_i$.
Hence, by monitoring the changes in $\hat{O}_i$, the receiver can determine the transmitted bits and extract $A_m$ from clock offsets. 
The above observations motivate our design of offset-based covert channels. 

% On CAN buses with heavy traffic, the noise in ITTs caused byarbitration can be very significant, and it would require a largeδvalue in order to establish a reliable ITT-based covert channel.Taking the message with ID=0x0C5 andT=10ms in the EcoCAR[1] as an example

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.48\columnwidth}
%         \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_offset_based_CC_0c5_IATs}
%         \caption{}
%         \label{fig:example_offset_based_CC_0c5_IATs}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.48\columnwidth}
%         \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_offset_based_CC_0c5_offsets}
%         \caption{}
%         \label{fig:example_offset_based_CC_0c5_offsets}
%     \end{subfigure}
%     \caption{Example message with ID=0x0C5 and a period of $T=10$ ms from the EcoCAR \cite{ecocar}. (a) The IATs vary between $9.3$ ms and $10.7$ ms. (b) Accumulated offsets. }
%     \label{fig:example_offset_based_CC_0c5}
% \end{figure}

\vspace{0.1cm}
\noindent \textbf{Embedding $A_m$ into ITTs.}
Different from the IAT-based covert channel (Section~\ref{sec:IAT_based_covert_channel}), the transmitter embeds each bit of $A_f$ into $L$ consecutive ITTs as follows,
\begin{equation*}
    \Delta t_j =
    \begin{cases}
        T - \delta, & \text{ if } b_i = 0,\\
        T + \delta, & \text{ if } b_i = 1,\\
        T, & \text{ else},
    \end{cases}
\end{equation*}
\rev{for $j \in [iL, (i+1)L),$} and 
\begin{equation*}
    \Delta t_j =
    \begin{cases}
        T + \delta, & \text{ if } b_i = 0,\\
        T - \delta, & \text{ if } b_i = 1,\\
        T, & \text{ else},
    \end{cases}
\end{equation*}
\rev{for $j \in [iL+L/2, (i+1)L)$}, where $L$ is assumed to be an even integer. 
In other words, in order to transmit a bit 0/1, the transmitter adds $-\delta$/$\delta$ to the first $L/2$ ITTs and then subtracts $-\delta$/$\delta$ from the following $L/2$ ITTs so that the observed clock offset returns to the reference level after the transmission of each bit.

\vspace{0.1cm}
\noindent \textbf{Extracting $A_m$ from Offsets.}
On the receiver side, the monitor node records the arrival timestamps and processes the IATs in batches. 
Since each $A_f$ has $n_f$ bits and each bit is modulated into $L$ consecutive ITTs, a total number of $N = n_f L$ consecutive IATs belong to the same $A_f$, where $N$ is referred to as the batch size. 

Denote the $i$-th IAT in the $k$-batch as $\Delta a_{k,i}$, where $1 \leq i \leq N$.  
Then the observed clock offset with respect to the beginning of the current batch up to the $i$-th IAT is 
\begin{equation*}
    \hat{O}_{k}[i] = iT - \sum_{j=1}^{i} \Delta a_{k,j}.
\end{equation*}
Let $\kappa = (\max(\hat{O}_{k}[i]) + \min(\hat{O}_{k}[i]))/2$ be the midpoint (assuming that at least a bit 0 and a bit 1 are transmitted), which is considered as the reference level of clock offsets.
\rev{Since clock skew is usually very small (100s of ppm) and we are computing batch-wise clock offsets, the impact of clock skew is small, and thus we assume that the $\kappa$ is constant for the duration of a batch\footnote{In the case of very large clock skew (e.g., 1000s of ppm), there will be a linear trend due to clock skew in batch-wise clock offsets and thus the reference level may not be constant. We leave the detrending process of clock offsets as future work.}.}
%, which is considered as the reference level of clock offsets\footnote{Note that since clock skew is usually very small (100s of ppm) and we are computing batch-wise clock offsets, the impact of clock skew is small. Hence, we assume that the (possibly non-zero) reference level is constant for the duration of a batch. Nevertheless, in the case of very large clock skew (e.g., 1000s of ppm), there will be a linear trend due to clock skew in batch-wise clock offsets and thus the reference level may not be constant. We leave the detrending process of clock offsets as future work.}. 
Since each bit affects $L$ IATs, the receiver needs to sample $\{\hat{O}_{k}[i]\}$ every $L$ values with a sampling offset of $\tau$ and obtain the $j$-th sample as $\hat{O}_{k}[jL + \tau]$. 
If $\tau$ is correctly chosen, then the total distance between each sample and the reference level should be maximized, i.e.,
\begin{equation*}
    \tau^* = \arg \max_{\tau} \sum_j | \hat{O}_{k}[jL + \tau] - \kappa|. 
\end{equation*}
Then the receiver converts the sampled values to bits through the following threhsolding-based scheme,
\begin{equation*}
    \hat{b}_j =
    \begin{cases}
        0, & \text{ if } \hat{O}_{k}[jL + \tau^*] > \Gamma_u,\\
        1,  & \text{ if } \hat{O}_{k}[jL + \tau^*] < \Gamma_l,\\
        \text{{\tt \_}}, & \text{ else, }%   // (Silence bit)}
    \end{cases}
\end{equation*}
where $\Gamma_l=\kappa - \frac{1}{4}\delta L$ and $\Gamma_u=\kappa + \frac{1}{4}\delta L$ are the lower and upper thresholds, respectively\rev{, and ``\_'' is the silence bit}. 
The term of $\frac{1}{4}\delta L$ is due to the fact that $\delta$ is added to (or subtracted from) $L/2$ consecutive ITTs, and thus the maximum total deviation is $\pm \frac{1}{2} \delta L$. 
The midpoints between $\kappa$ and $\kappa \pm \frac{1}{2} \delta L$ are chosen as thresholds. 
Eventually, $A_m$ is extracted by concatenating all decoded bits and splitting them at the silence bits. 

\vspace{0.1cm}
\noindent \textbf{Impact on CAN bus schedulability.} As we have shown, in both the IAT-based and offset-based covert channels, a certain amount of deviation is added to the ITTs.
As a result, it may increase the worst-case response time of CAN messages, which is defined as the longest time from the initiating event (that puts the message in the transmission queue) occurring to the message being received by the nodes that require it.
If we apply the schedulability analysis in \cite{davis2007controller} to TACAN, we can show that the effect of TACAN is equivalent to increasing the blocking delay by a constant amount of time (hundreds of $\mu$s) and increasing the message transmission time by a small percentage. 
Therefore, to achieve effective use of covert channels, TACAN parameters need to be experimentally obtained and fine tuned prior to deployment to ensure the schedulability of the CAN bus.
%to ensure the schedulability of the CAN bus.
A more detailed discussion is provided in Appendix~\ref{appendix:schedulability}.


\new{Generalize this approach to messages with large clock skew}

==> TACAN Extension (arXiv)/Sections/Bio.tex <==
\balance
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Bio/xuhang-ying}}]{Xuhang Ying}
	(S'15) is a Postdoctoral Research Associate at the Network Security Lab at University of Washington. 
	He received his B.Eng. degree in Information Engineering from the Chinese University of Hong Kong, his M.S. and Ph.D. degrees in Electrical Engineering from the University of Washington in 2013, 2016, and 2018, respectively. 
	His Ph.D. research focused on crowdsensing and resource allocation in shared spectrum. 
	His research interests include Controller Area Networks (CAN) security and wireless security.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/giuseppe}}]{Giuseppe Bernieri}
is a Postdoctoral Researcher at the Department of Mathematics, University of Padua, Padua, Italy. He received the Ph.D. degree in computer science and automation from the University of Roma Tre, Rome, Italy. His research interests include cyber-physical system security, cyber security applied to industrial control systems and critical infrastructures, the development and the implementation of ad-hoc solutions for the detection of cyber-physical threats affecting SCADA systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/mauro}}]{Mauro Conti}
is Full Professor at the University of Padua, Italy. He obtained his Ph.D. from Sapienza University of Rome, Italy, in 2009. After his Ph.D., he was a Post-Doc Researcher at Vrije Universiteit Amsterdam, The Netherlands. In 2011 he joined as Assistant Professor the University of Padua, where he became Associate Professor in 2015, and Full Professor in 2018. He has been Visiting Researcher at GMU (2008, 2016), UCLA (2010), UCI (2012, 2013, 2014, 2017), TU Darmstadt (2013), UF (2015), and FIU (2015, 2016). He has been awarded with a Marie Curie Fellowship (2012) by the European Commission, and with a Fellowship by the German DAAD (2013). His research is also funded by companies, including Cisco and Intel. His main research interest is in the area of security and privacy. In this area, he published more than 200 papers in topmost international peer-reviewed journals and conference. He is Associate Editor for several journals, including IEEE Communications Surveys \& Tutorials, IEEE Transactions on Information Forensics and Security, and IEEE Transactions on Network and Service Management. He was Program Chair for TRUST 2015, ICISS 2016, WiSec 2017, and General Chair for SecureComm 2012 and ACM SACMAT 2013. He is Senior Member of the IEEE.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/Bushnell}}]{Linda Bushnell}(F'17)
	is a Research Professor and the Director of the Networked Control Systems Lab in the Electrical and Computer Engineering Department at the University of Washington - Seattle. She received the B.S. degree and M.S. degree in Electrical Engineering from the University of Connecticut - Storrs in 1985 and 1987, respectively. She received the M.A. degree in Mathematics and the Ph.D. degree in Electrical Engineering from the University of California - Berkeley in 1989 and 1994, respectively. Her research interests include networked control systems, control of complex networks, and secure-control. She was elected a Fellow of the IEEE for her contributions to networked control systems. She is a recipient of the US Army Superior Civilian Service Award, NSF ADVANCE Fellowship, and IEEE Control Systems Society Distinguished Member Award. She is currently an Associate-Editor for \emph{Automatica} and \emph{IEEE Transactions on Control of Network Systems} and Series Editor for the Springer series \emph{Advanced Textbooks in Control and Signal Processing.} 
	She is currently Chair of the IEEE Control Systems Society (CSS) Women in Control Standing Committee, and Liaison to IEEE Women in Engineering (WIE). She is also the Treasurer of the American Automatic Control  Council (AACC) and a Member of the International Federation of Automatic Control (IFAC) Technical Board.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bio/Poovendran}}]{Radha Poovendran}(F'15)
	is a Professor and the Chair of the Electrical and Computer Engineering Department at the University of Washington (UW). He is the Director of the Network Security Lab (NSL) at the University of Washington. He is the Associate Director of Research of the UW Center for Excellence in Information Assurance Research and Education. He received the B.S. degree in Electrical Engineering and the M.S. degree in Electrical and Computer Engineering from the Indian Institute of Technology- Bombay and University of Michigan - Ann Arbor in 1988 and 1992, respectively. He received the Ph.D. degree in Electrical and Computer Engineering from the University of Maryland - College Park in 1999. His research interests are in the areas of wireless and sensor network security, control and security of cyber-physical systems, adversarial modeling, smart connected communities, control-security, games-security and information theoretic security in the context of wireless mobile networks. He is a Fellow of the IEEE for his contributions to security in cyber-physical systems. He is a recipient of the NSA LUCITE Rising Star Award (1999), National Science Foundation CAREER (2001), ARO YIP (2002), ONR YIP (2004), and PECASE (2005) for his research contributions to multi-user wireless security. He is also a recipient of the Outstanding Teaching Award and Outstanding Research Advisor Award from UW EE (2002), Graduate Mentor Award from Office of the Chancellor at University of California - San Diego (2006), and the University of Maryland ECE Distinguished Alumni Award (2016). He was co-author of award-winning papers including IEEE/IFIP William C. Carter Award Paper (2010) and WiOpt Best Paper Award (2012). He holds eight patents in wireless and aviation security.
\end{IEEEbiography}

==> TACAN Extension (arXiv)/Sections/acknoledgments.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi

The authors would like to thank...

==> TACAN Extension (arXiv)/Sections/appendices.tex <==
\newpage

\balance
\appendices
% \section{CAN Frame}
% \label{appendix:CAN_frame}
% As illustrated in Figure~\ref{fig:can_frame_structure}, each CAN frame or message has a set of predefined fields, including the Start of Frame (SOF) field, the Arbitration field (including a 11-bit message ID for the base frame format or a 29-bit message ID for the extended frame format), the Control field, the Data field (8-64 bits), the CRC field, the ACK field, and the End of Frame (EOF) field.

% \begin{figure}[ht!]
% \centering
% \includegraphics[width=1\columnwidth]{./Figures/can_frame_structure}
% \caption{Illustration of CAN frame structure.}
% \label{fig:can_frame_structure}
% \vspace{-0.3cm}
% \end{figure}

\section{Impact on CAN Bus Schedulability}
\label{appendix:schedulability}
In order to understand the impact of the timing parameter $\delta$ introduced by the IAT-based covert channel in TACAN on CAN bus schedulability, we apply the schedulability analysis in \cite{davis2007controller}.
For the ease of discussion, we provide a summary of definitions as below. 
%The same notations in \cite{davis2007controller} are used for consistency.
\begin{itemize}
    \item $k$: Message priority, which is used interchangeably with the message ID.
    \item $C_k$: Transmission time, defined as the longest time that the message can take to be transmitted.
    \item $J_k$: Queuing jitter, defined as the longest time between the initiating event and the message being queued, ready to be transmitted on the bus.
    \item $w_k$: Queuing delay, defined as the longest time that the message can remain in the CAN controller slot or device driver queue, before commencing successful transmission on the bus.
    \item $T_k$: Message period, defined as the minimum inter-arrival time of the event that triggers queueing of the message. 
    Such events may occur strictly periodically with a period of $T_k$ or sporadically with a minimum separation of $T_k$. 
    \item $R_k$: Worst-case response time of message $k$, defined as the longest time from the initiating event occurring to the message being received by the nodes that require it.
    \item $D_k$: Hard deadline, defined as the maximum permitted time from occurrence of the initiating event to the end of successful transmission of the message. 
\end{itemize}
A message is \textit{schedulable} if and only if its worst-case response time is no greater than its deadline ($R_k \leq D_k$). 
A CAN bus is schedulable if and only if all messages on the CAN bus are schedulable.

As per \cite{davis2007controller}, we have $C_k = (80 + 10 s_k)\tau_{bit}$ (including bit stuffing), where $s_k$ is the number of data bytes and $\tau_{bit}$ is the transmission time of a single bit. 
For a $8$-byte message on a $500$ kbps CAN bus, we have $\tau_{bit}=2~\mu$s and  $C_k=320$ $\mu$s.
While CAN nodes typically have separate clock sources, all the timing quantities (e.g., message jitters, bit times, message periods, and deadlines) that derived from node clocks will be converted to real-time. 

The message $k$'s worst-case response time $R_k$ is given by
\begin{equation*}
    R_k = J_k + w_k + C_k,
\end{equation*}
and the queuing delay $w_k$ consists of two elements:
\begin{itemize}
    \item \textit{Blocking} $B_k$, due to lower priority messages  being transmitted when message $k$ is queued, and
    \item \textit{Interference} due to higher priority messages which may win arbitration and be transmitted in preference to message $k$.
\end{itemize}
The blocking delay is given by $B_k = \max_{i \in lp(k)} (C_i)$, where $lp(k)$ is the set of messages with lower priority than $k$.

In order to analyze the worst-case response time, it is important to characterize the busy period, where all messages of priority $k$ or higher, queued strictly before the end of busy period, are transmitted during the busy period. 
The maximal busy period begins with a so-called critical instant where message $k$ is queued simultaneously with all higher priority messages and then each of these higher priority messages is subsequently queued again after the shortest possible time interval.

For simplicity, we assume that only one instance of message $k$ is transmitted during a priority level-$k$ busy period. 
In this case, the worst-case queuing delay is 
\begin{equation}\label{eq:worst_case_queuing_delay}
    w_k = B_k + \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k + J_i + \tau_{bit}}{T_i}  \right\rceil C_i.
\end{equation}
Since the right hand side is a monotonic non-decreasing function of $w_k$, Eq.~(\ref{eq:worst_case_queuing_delay}) can be solved using the following recurrence relation,
\begin{equation}\label{eq:worst_case_queuing_delay2}
    w_k^{n+1} = B_k + \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k^n + J_i + \tau_{bit}}{T_i} \right\rceil C_i.
\end{equation}
A suitable starting value is $w_k^0 = B_k$, and the recurrence relation iterates until, either $J_k + w_k^{n+1} + C_k > D_k$, i.e., the message is not schedulable, or $w_k^{n+1}=w_k^n$, in which case the worst-case response of message $k$ is given by $J_k + w_k^{n+1}+C_k$. 

In order to apply the above schedulability analysis to TACAN, we define $T'_k = T_k - \delta$. 
Since TACAN adds at most $\delta$ to each ITT, which can be considered as part of the queuing jitter, we have $J'_k=J_k + \delta$. 
Assume that $\delta = 0.01 T_k$ and all messages employ the IAT-based covert channel. 
By substituting $T'_k=0.99 T_k$ and $J'_m=J_m + 0.01 T_k$ into Eq.~(\ref{eq:worst_case_queuing_delay2}), we have
\begin{align}
    w_k^{' n+1} &= B_k + \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k^{' n} + (J_i + 0.02 T_i) + \tau_{bit}}{0.98 T_i} \right\rceil C_i \nonumber\\
    &\approx B'_k  + 
    \sum_{\forall i \in hp(k)} \left\lceil \frac{w_k^{' n} + J_k + \tau_{bit}}{T_i} \right\rceil C'_i, \label{eq:updated_worst_case_queuing_delay}
\end{align}
where 
\begin{equation}\label{eq:appendix:blocking_delay}
    B_k' = B_k + \sum_{\forall i \in hp(k)} \left(\frac{0.01}{0.99} C_i \right), 
\end{equation}
and 
\begin{equation}\label{eq:appendix:msg_tx_time}
    C'_i = \frac{1}{0.99} C_i = 1.01 C_i.
\end{equation}
Therefore, the impact of $\delta$ on the worst-case response time is threefold: 1) increasing the queuing jitter by a fixed amount of time, 2) increasing the blocking delay by a bounded amount of time, and 3) increasing the equivalent message transmission time of higher priority messages by a certain percentage.

As an example, let us consider a 10-ms message and set $\delta=0.01T=0.1$ ms. 
Then the increase in the queuing jitter is $100~\mu$s. 
Assuming 45 higher priority messages (half of the messages on the EcoCAR \cite{ecocar}) with 8-byte data on a 500 kbps bus ($C_i=320~\mu$s), the increase in the blocking delay is $145~\mu$s (Eq.~(\ref{eq:appendix:blocking_delay})). 
In addition, the equivalent increase in the message transmission time of each higher priority message is $1\%$, which is equal to $3.2~\mu$s (Eq.~(\ref{eq:appendix:msg_tx_time})). 
By solving Eq.~(\ref{eq:updated_worst_case_queuing_delay}), we can compute the corresponding worst-case response time of message $k$ with TACAN. 
%The above discussion suggests that schedulability tests will need to be performed during TACAN configurations to ensure the schedulability of the system.
Hence, to achieve effective use of covert channels, the TACAN parameter $\delta$ needs to be experimentally obtained and fine tuned prior to deployment to ensure the schedulability of the CAN bus.



==> TACAN Extension (arXiv)/Sections/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> TACAN Extension (arXiv)/Sections/conclusion.tex <==
\section{Conclusion}
%\section{Conclusion} 
\label{sec:conclusion}
In this paper, we presented TACAN, a covert channel-based transmitter authentication scheme that allows a MN to verify the authenticity of the transmitting ECU. 
We developed IAT-based, LSB-based, and hybrid covert channels to communicate the authentication information between ECUs and the MN without introducing protocol modifications or traffic overheads. 
We analytically modeled the bit error probability of the IAT-based covert channel as a function of covert channel parameters, and studied its impact on the CAN bus schedulability. 
We experimentally validated and evaluated TACAN and the proposed channels using the EcoCAR testbed and the publicly available Toyota dataset.
Our results show that properly configured IAT-based covert channels have an experimental bit error probabilities of less than 0.3\%. 
We also show that our TACAN-based detector can detect CAN bus attacks with a high detection probability, while keeping the false alarm probability less than 0.33\% by setting the detection threshold to $2$ or higher. 
In addition, we studied the impact of the LSB-based covert channel on sensor values and observed moderate accuracy loss. 

%We provided a security discussion for TACAN and demonstrated the proposed covert channels through testbed validation and experimental evaluation.
%Our future work will include experimental evaluation of TACAN under various attacks against the CAN bus.
%In addition, we will also improve the throughput of the proposed covert channels and explore hybrid covert channel schemes.

%In future works we will address complex attacks implementation to evaluate the authentication methodologies conceived. Moreover, we will extend the covert channels schemes considering simultaneously exploitation of time-based and storage-based to improve our proposal.

%\cmt{Shaun: Add future work?}

% As future work, we will 

% \giuseppe{evaluation of multiple kind of CAN messages will be provided in the future works}

% We will combine the authentication messages embedding methodologies to better address authentication requirements and improve the overall technique.

% Future work:
% \begin{itemize}
%     \item Implement real-time receiver; sequence generation and verification. 
% \end{itemize}

==> TACAN Extension (arXiv)/Sections/discussion.tex <==
\section{Discussion}
\shaun{Should we keep this section or not?}

\subsection{Impact of Missing Messages}

\subsection{Use of Error Correction Code}
When the probability of bit errors is reasonably small, one may also consider Error Correction Coding (ECC) techniques that are widely used in communications \cite{goldsmith2005wireless} to detect and recover occasional bit errors. 
\rev{Nevertheless, the use of ECC techniques will unavoidably complicates the design of covert channels and introduces overheads.
In addition, since the probability of consecutive corrupted authentication frames is small, it is acceptable to not recover the bit errors in a particular frame.}

\subsection{Detection Delays}

\subsection{A Communication Channel Perspective}
How to improve channel throughput? 

Tradeoff between throughput and length 

\begin{itemize}
    \item Capacity
    \item Non-return-to-zero (NRZ)
    \item Error correction code
    \item Multiple levels
    \item CRC
\end{itemize}

==> TACAN Extension (arXiv)/Sections/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
In this section, we conduct extensive experiments to evaluate the performance of the proposed covert channels and TACAN using real-world datasets. 
We first describe our real vehicle CAN bus testbed based on the UW EcoCAR (a Chevrolet Camaro 2016) and demonstrate the proposed IAT-based and LSB-based covert channels (Section~\ref{sec:eval:testbed_validation}). 
We then evaluate the bit error performance (Section~\ref{sec:eval:bit_error}), throughput (Section~\ref{sec:eval:throughput}), detection performance (Section~\ref{sec:eval:detection}), and accuracy loss (Section~\ref{sec:eval:accuracy_loss}) of TACAN using the EcoCAR datatset as well as the publicly available Toyota dataset collected from the Toyota Camry 2010 \cite{toyota2010dataset}. 

\subsection{Testbed Validation} 
\label{sec:eval:testbed_validation}
Fig.~\ref{fig:testbed_setup} illustrates our EcoCAR testbed that consists of the UW EcoCAR and testbed ECUs, which are connected via the On-Board Diagnostics (OBD-II) port
The EcoCAR hosts 8 stock ECUs and two experimental ECUs.
A total of 2500+ messages with 89 different IDs are exchanged on the CAN bus every second.
All messages are periodic with periods ranging from 10 ms to 5 sec. 

Each testbed ECU consists of a Raspberry Pi 3 and a PiCAN 2 board (using a MCP2515 CAN controller and a MCP2551 CAN transceiver). 
The Raspberry Pi-based ECU is programmed to be a receive-only device that records CAN messages using SocketCAN \cite{socketCAN}.
During data collection, the EcoCAR is in the park mode in an isolated and controlled environment for safety purposes, but all in-vehicle ECUs are functional and actively exchange CAN messages. 
%The Camry Toyota 2010 dataset \cite{toyota2010dataset} consists of 43 distinct messages, and the majority of them are periodic with periods ranging from 10 ms to 5 sec.


\begin{figure}[t!]
\centering
\includegraphics[trim=0cm 0.4cm 0cm -0.5cm,clip=true,width=1\columnwidth]{./Figures/testbed_setup}
\caption{Illustration of  EcoCAR testbed. Raspberry Pi-based testbed ECUs are connected to the OBD-II port at the back of the EcoCAR.%, one as the transmitter and the other one as the receiver.
}
\label{fig:testbed_setup}
\end{figure}


% \rev{Table~\ref{table:representative_messages} lists five representative messages with different IDs and periods from the EcoCAR and toyota datasets. 
% To quantify the noise level, we consider the standard deviation and the range (the difference between the maximum and the minimum) of IATs, both of which are normalized by the message period. 
% We observe a significant difference in the noise level among CAN messages within the same vehicle, which implies a need for customized settings for the IAT-based covert channel.}

% \begin{table}[h!]
%     \footnotesize
% 	\centering
% 	\caption{Statistics of IATs of representative messages from the Toyota dataset and the EcoCAR testbed.}
% 	\label{table:representative_messages}
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%     \multirow{2}{*}{Msg ID} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Period\\ (sec)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Standard dev.\\ (Normalized)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Range\\ (Normalized)\end{tabular}} & \multirow{2}{*}{Source} \\
%      &  &  &  &  \\ \hline
%     0x020 & 0.01 & 1.1\% & 10.2\% & Toyota \\ \hline
%     0x0B4 & 0.02 & 0.5\% & 4.6\% & Toyota \\ \hline 
%     0x224 & 0.03 & 0.9\% & 4.8\% & Toyota \\ \hline
%     0x620 & 0.3 & 1.0\% & 65.3\% & Toyota \\ \hline
%     0x0D1 & 0.01 & 2.7\% & 51.5\% & EcoCAR \\ \hline
%     %0x180 & 10 & 1.7\% & 30.1\% & EcoCAR \\ \hline
%     0x185 & 0.02 & 1.3\% & 22.6\% & EcoCAR \\ \hline
%     0x22A & 0.1 & 1.2\% & 6.4\% & EcoCAR \\ \hline
%     \end{tabular}
%     \normalsize
% \end{table}



To demonstrate the proposed IAT-based and LSB-based covert channels, we use the testbed ECU to record the timestamps of 100-ms message 0x22A from the EcoCAR testbed and replay them in our experiments. 
In the ideal case, the TACAN transmitter will add $\pm \delta$ to the ITTs, which correspond to changes of $\pm \delta/(1+S)$ at the receiver side. 
Since both $\delta$ and $S$ are very small, we approximate $\delta/(1+S)$ as $\delta$ and program the TACAN transmitter to directly modify the recorded IATs. 


Fig.~\ref{fig:example_of_iat_based_covert_channel_0x22a_ecocar} provides an example of the received authentication frame in the IAT-based covert channel.
In this example, the 24-bit counter has a value of 1, $\delta = 0.01T$, and $L=4$. 
We observe that without the running average, the received IATs can be very noisy, which leads to possible bit errors, whereas computing running averages can effectively smooth out the noise. 
We also observe that the actual length of the transmitted frame can exceed the original length due to the inserted stuffed bits.


\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=0cm 0.4cm 0cm 0cm,clip=true,width=1\textwidth]{Figures/example_of_iat_based_covert_channel_0x22a_ecocar}
        \caption{IAT-based covert channel}
        \label{fig:example_of_iat_based_covert_channel_0x22a_ecocar}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=-0.8cm 0.4cm 0.4cm 0cm,clip=true,width=.98\textwidth]{Figures/example_of_lsb_based_covert_channel_0x22a_ecocar}
        \caption{LSB-based covert channel}
        \label{fig:example_of_lsb_based_covert_channel_0x22a_ecocar}
    \end{subfigure}
    \caption{Example of received authentication frame for message 0x22A from the EcoCAR testbed in (a) the IAT-based covert channel and (b) the LSB-based covert channel. The fields for SOF, counter and digest values (Data), CRC, and EOF are colored in blue, green, gray, yellow, and red, respectively. The stuffed bits are marked as black triangles. %\shaun{(Shaun: background colors are not visible when printed in black and white. Do we still want to keep it?)}
    } 
    \label{fig:example_of_covert_channel_0x22a}
\end{figure}

Fig.~\ref{fig:example_of_lsb_based_covert_channel_0x22a_ecocar} provides an example of the received authentication frame in the LSB-based covert channel when a single LSB is used ($L=1$).
Compared to the IAT-based covert channel in Fig.~\ref{fig:example_of_iat_based_covert_channel_0x22a_ecocar}, the LSB-based covert channel is noise-free, and each authentication frame can be transmitted in a shorter duration. 

\subsection{Bit Error Performance}
\label{sec:eval:bit_error}
In this section, we discuss the bit error performance of the IAT-based and LSB-based covert channels. 
In addition to the EcoCAR dataset, we also use the Camry Toyota 2010 dataset \cite{toyota2010dataset}.
It consists of 43 distinct messages, and the majority of them are periodic with periods ranging from 10 ms to 5 sec.


\vspace{0.1cm}
\noindent \textbf{IAT-based covert channel.}
In this experiment, we select a subset of 9 representative messages from the Toyota dataset and the EcoCAR testbed with different message ID levels, periods, and noise levels, as listed in Table~\ref{table:representative_messages}. 
Our objective is to compare the analytical bit error probabilities ($P_e$) in Eq.~(\ref{eq:bit_error_probability}) against the experimental values and study the impact of $L$. 
We set $\delta =0.01T$ to minimize the impact on the CAN bus.  
Since $P_e$ is a function of the standard deviation of IATs $\sigma$ (Eq.~(\ref{eq:bit_error_probability})), we only consider IATs within $\pm 20\%$ of the average when computing $\sigma$ to minimize the adverse impact of outliers. 
To obtain the experimental $P_e$, we add $\pm \delta$ to the IATs and compute the running averages of window length $L$. 
We then compute the percentage of the averaged IATs that lead to bit errors as the experimental $P_e$. 


\begin{table}[t!]
    \footnotesize
	\centering
	\caption{Statistics of IATs of representative messages from the Toyota dataset and the EcoCAR testbed.}
	\label{table:representative_messages}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \multirow{2}{*}{Msg ID} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Period\\ (sec)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Standard deviation\\ (Norm. by period)\end{tabular}} & \multirow{2}{*}{Source} \\
     &  &  &   \\ \hline
    0x020 & 0.01 & 1.1\% & Toyota \\ \hline
    0x0B4 & 0.02 & 0.5\% & Toyota \\ \hline 
    0x224 & 0.03 & 0.9\% & Toyota \\ \hline
    0x620 & 0.3 & 1.0\% & Toyota \\ \hline
    0x0D1 & 0.01 & 2.7\% & EcoCAR \\ \hline
    %0x180 & 0.01 & 1.7\% & EcoCAR \\ \hline
    0x185 & 0.02 & 1.6\% & EcoCAR \\ \hline
    0x22A & 0.1 & 1.2\% & EcoCAR \\ \hline
    0x3FB & 0.25 & 1.4\% & EcoCAR \\ \hline
    0x4D1 & 0.5 & 1.4\% & EcoCAR \\ \hline
    \end{tabular}
    \normalsize
    %\vspace{0.3cm}
\end{table}

As shown in Fig.~\ref{fig:bit_error_prob}, the bit error performance of the IAT-based covert channel varies a lot among different messages. 
In general, $P_e$ is very high with $L= 1$, but it quickly drops to as $L$ increases for all messages, which  demonstrates the effectiveness of the running average. 
For the four Toyota messages, the experimental $P_e$ is less than $0.1\%$ with $L=3$, and the experimental $P_e$ is less than $0.3\%$ with $L=5$ for the five EcoCAR messages. 
In addition, since the EcoCAR has significantly more traffic than the Toyota Camry, we observe larger $P_e$ for EcoCAR messages than those for the Toyota messages for the same $L$.
We also observe that since we set $\delta$ to a fixed percentage of the message period, messages with larger periods tend to be more advantageous and usually have a smaller $P_e$ with the same $L$. 

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=0cm 0.5cm 0cm 0cm,clip=true,width=1\textwidth]{Figures/bit_error_prob_toyota}
        \caption{Toyota dataset}
        \label{fig:bit_error_prob_toyota}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=0cm 0.5cm 0cm 0cm,clip=true,width=1\textwidth]{Figures/bit_error_prob_ecocar}
        \caption{EcoCAR testbed}
        \label{fig:bit_error_prob_ecocar}
    \end{subfigure}
    \caption{Comparison of analytical and experimental bit error probabilities for selected messages from (a) the Toyota dataset and (b) the EcoCAR testbed. We observe that increasing $L$ will reduce the bit error probability. We also obesrve that our analysis provides a good estimate of the experimental bit error probability.
    } 
    \label{fig:bit_error_prob}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=1\columnwidth]{./Figures/hist_L_ecocar}
\caption{Histogram of $L_{\min}$ such that $P_e \leq 1\%$ for EcoCAR messages with $\delta=0.01T$.
}
\label{fig:hist_L_ecocar}
\end{figure}

In order to further understand the minimum $L$ values required by different messages, we choose 85 EcoCAR messages and determine $L_{\min}$ such that the experimental bit error probability is less than or equal to $1\%$ with $\delta = 0.01T$.
Note that we exclude four noisy messages, each of which has a standard deviation of IATs that is $10\%$ larger than its mean IAT. 
%Hence, we consider them as noisy messages that are not suitable for IAT-based covert channel deployment. 
As shown in Fig.~\ref{fig:hist_L_ecocar}, a total of 19 messages can use $L=1$.
With $L\leq 5$, a total of 46 messages are eligible, accounting for $51.7\%$ of EcoCAR messages. 
If we set $\delta=0.02T$, a total of 59 messages become eligible, which corresponds to $66.3\%$ of all messages. 

\vspace{0.1cm}
\noindent \textbf{LSB-based covert channel.}
Since the authentication message is hidden in a few bits of the data payload of normal CAN messages in the LSB-based covert channel, the bit error probability will be as low as that of the CAN bus itself. 
According to~\cite{ferreira2004experiment}, the bit error probability of the CAN bus in normal environments (factory production line) and aggressive environments (two meters away from a high-frequency arc-welding machine) are $3.1\times 10^{-7}\%$ and $2.6 \times 10^{-5}\%$, respectively.
In other words, the LSB-based covert channel is very reliable and is not affected by the noise caused by the CAN traffic. 

\subsection{Throughput Performance}
\label{sec:eval:throughput}
In this section, we compute and compare the throughput of the proposed covert channels. 
For ease of discussion, we let the number of bits in the authentication message ($A_m$) be $N_m$, and the number of bits in other fields (SOF, CRC, and EOF) be $N_o$. 
Hence, each authentication frame (denoted as $A_f$) has $N_f = N_m + N_o$ bits. 
However, the number of actually transmitted bits may be more than $N_f$ due to bit stuffing. 
Since the stuffed bit itself may be the first of the five consecutive identical bits, there is at most one stuffing bit every four original bits after the first one. 
Therefore, the actual length of each frame is bounded by
\begin{equation*}
    N'_{f} = N_f + \left\lfloor \frac{N_f - 7 - 1}{4} \right\rfloor, \label{eq:worst_case_frame_size}
\end{equation*}
where $\lfloor \cdot \rfloor$ is the floor function.
Note that we need the $-7$ in the numerator because the EOF is not subject to bit stuffing, and the $-1$ is because the worst-case bit stuffing happens right after the first original bit.  

To quantify the throughput performance, we define two metrics: 1) channel throughput ($R_c$), i.e., the number of bits transmitted per second, and 2) authentication throughput ($R_a$), i.e., the number of authentication bits transmitted per second. 
Since the clock skew is very small and its effect is usually negligible, it is omitted to simplify calculations.

\vspace{0.1cm}
\noindent \textbf{IAT-based covert channel.}
Since every bit is embedded into $L$ consecutive ITTs of $T$ sec, it takes $LT$ time to transmit one bit, which means $R_c = 1/(LT)$. 
The best-case authentication throughput (without bit stuffing) is $R_a=N_m/(N_fLT)$. 
With bit stuffing, $R_a$ may be as low as $N_m/(N'_fLT)$.

\vspace{0.1cm}
\noindent \textbf{LSB-based covert channel.}
Since up to $L$ authentication bits can be hidden in one CAN message, we have $R_c = L/T$. 
Each frame requires $\lceil N_f/L \rceil$ normal CAN messages and a duration of $\lceil N_f/L \rceil T$ to transmit.
Hence, we have $R_c = N_m/(\lceil N_f/L \rceil T) \approx N_mL/(N_fT)$ in the best case and $R_c=N_mL/(N'_fT)$ in the worst case. 

\vspace{0.1cm}
\noindent \textbf{Hybrid covert channel.}
As presented in Section~\ref{sec:hybrid}, the hybrid covert channel splits $A_m$ into two parts with a suitable splitting ratio of $\alpha$ (Eq.~(\ref{eq:splitting_ratio})) and transmits them through the IAT-based and LSB-based covert channels separately. Let $D=\max((\lceil\alpha N_m \rceil + N_o)L_1,  (\lceil(1-\alpha) N_m \rceil + N_o) /L_2)$ be the time it takes to transmit a single frame.
Hence, the channel throughput is $R_c = (N_m+2N_o)/D$. 
%, where $L_1$ is the number of LSBs in the LSB-based covert channel. 
The best-case authentication throughput is 
%$R_a = N_m/((\lceil(1-\alpha) N_m \rceil + N_o) /L)$. 
$R_a = N_m/D$.
% The authentication throughput gain over the LSB-based covert channel (which has a higher authentication throughput than the IAT-based covert channel) is 
% \begin{equation*}
%     \frac{\alpha N_m}{((1-\alpha)N_m+N_o)/L_2 - 1}\times 100\%. \label{eq:throughput_gain}
% \end{equation*}. 

\vspace{0.1cm}
\noindent \textbf{Throughput comparison.}
In this experiment, we consider a 10-ms CAN message and set $N_m=32$ and $N_o=16$. 
The average throughput is computed for each covert channel for transmitting $1000$ authentication frames. 
Results are provided in Table~\ref{table:throughput_comparison}. 
We can see that $R_c$ of the hybrid covert channel is close to the sum of $R_c$ of individual covert channels, but they are not exactly equal due to bit stuffing.
When $L_1=L_2=1$, the hybrid covert channel has a gain of $49.7\%$ in $R_a$ over individual covert channels.
As either $L_1$ or $L_2$ increases, the throughput of the IAT-based covert channel becomes smaller than that of the LSB-based covert channel, and it is less beneficial to deploy the hybrid covert channel. %In addition, as the message period increases, the throughput of all covert channels will decrease proportionally. 
With $L_1=L_2=2$, the hybrid covert channel reduces to the LSB-based covert channel, because no authentication bits are transmitted over the IAT-based covert channel.

\begin{table}[h!]
\caption{Comparison of throughput (in bits per second) of three proposed covert channels with 10-ms CAN messages}
\label{table:throughput_comparison}
\begin{tabular}{|c|c|c||c|c||c|c|}
\hline
\multirow{2}{*}{\textbf{Settings}} & \multicolumn{2}{c||}{\textbf{IAT-Based}} & \multicolumn{2}{c||}{\textbf{LSB-Based}} & \multicolumn{2}{c|}{\textbf{Hybrid}} \\ \cline{2-7} 
 & $R_c$ & $R_a$ & $R_c$ & $R_a$ & $R_c$ & $R_a$ \\ \hline
$L_1=1, L_2=1$ & 100.0  & 61.8 & 100.0  & 61.8 & 198.6  & 92.5 \\ \hline
$L_1=2, L_2=1$ & 50.0 & 30.9 & 100.0 & 61.8 & 148.8 & 69.3 \\ \hline
$L_1=1, L_2=2$ & 100.0 & 61.8  & 197.8 & 122.3 & 296.7 & 138.1 \\ \hline
% $L_1=2, L_2=2$ & 50.0  & 30.9 & 200.0  & 123.6 & 199.1 & 123.1 \\ \hline
$L_1=2, L_2=2$ & 50.0  & 30.9 & 197.8 & 122.3 & 197.8 & 122.3 \\ \hline
\end{tabular}
\end{table}


\subsection{Detection of CAN Bus Attacks}
\label{sec:eval:detection}
As described in Section~\ref{sec:proposed_scheme}, TACAN extracts and verifies the authentication message embedded in the IATs or LSBs of normal CAN messages to authenticate the transmitting ECU and also serves the purpose of intrusion detection.
In this section, we consider a TACAN-based detector and evaluate its detection performance against CAN bus attacks.
While we focus on the IAT-based covert channel,  similar results can be found in the other two covert channels.

\vspace{0.1cm}
\noindent \textbf{Detection scheme.}
The TACAN-based detection scheme works as follows: the MN counts the number of consecutive authentication failures.
An authentication failure is either a message reception failure (e.g., lost message, CRC error) or a message verification failure (e.g., invalid counter or digest).
If the counter is larger than or equal to a preset threshold $K$ (e.g., $K=3$), then the MN raises an alert for a CAN bus attack. A successfully received and verified authentication message will reset the detection counter to zero. 

%In the rest of this section, we will show how this TACAN-based detector can identify attacks that interrupt the transmission of normal CAN messages (e.g., suspension and injection attacks), as well as attacks in which attackers fail to generate valid authentication messages (e.g., forgery, replay, and masquerade attacks).

% \begin{table}[t!]
% \caption{Authentication message reception in the IAT-based covert channel in the normal situation}
% \label{table:message_reception_normal}
% \centering
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{Msg ID} & \textbf{Total} & \textbf{Lost} & \textbf{\begin{tabular}[c]{@{}c@{}}CRC\\ Errors\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Correctly\\ Received\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Success \\ Rate (\%)\end{tabular}} \\ \hline
% 0x0D1 & 2604 & 10 & 3 & 2591 & 99.50 \\ \hline
% 0x185 & 1292 & 9 & 8 & 1275 & 98.68 \\ \hline
% 0x22A & 772 & 0 & 0 & 772 & 100.00 \\ \hline
% 0x3FB & 308 & 2 & 0 & 0 & 99.35 \\ \hline
% 0x4D1 & 154 & 2 & 0 & 1 & 98.05 \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[]
\caption{False alarm probability in the IAT-based covert channel in the normal situation}
\label{table:false_alarm_prob_normal}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Msg ID} & \textbf{$K=1$} & \textbf{$K=2$} & \textbf{$K=3$} \\ \hline
0x0D1 & 0.49\% & 0.19\% & 0.0\% \\ \hline
0x185 & 1.31\% & 0.31\% & 0.0\% \\ \hline
0x22A & 0.0\% & 0.0\% & 0.0\% \\ \hline
0x3FB & 0.64\% & 0.32\% & 0.0\% \\ \hline
0x4D1 & 1.95\% & 0.33\% & 0.0\% \\ \hline
\end{tabular}
\end{table}

\vspace{0.1cm}
\noindent \textbf{False alarm probability.}
We first discuss the false alarm probability (denoted as $P_{FA}$) of the TACAN-based detector, which is defined as the probability of raising an alarm when there is no attack present. 
We experimentally evaluate the IAT-based covert channel in the normal situation using the five CAN messages from the EcoCAR testbed (see Table~\ref{table:representative_messages}).
An example of the normal IAT-based covert channel transmission is provided in Fig.~\ref{fig:example_of_iat_based_covert_channel_normal}.
In order to minimize bit errors, we set $\delta=0.02T$ and set $L=6$ for the first three messages and set $L=2$ for the last two messages.

As shown in Table~\ref{table:false_alarm_prob_normal}, with a properly configured IAT-based covert channel, we have $P_{FA} \leq 2\%$ with $K=1$. 
When $K=2$, we have $P_{FA} \leq 0.33\%$ for all messages. 
Since none of the messages has three consecutive message reception failures (either a lost message or a CRC error), we have $P_{FA}=0\%$ with $K=3$. 
Note that since the LSB-based covert channel has a very low bit error probability, the probability of a message reception failure in the normal situation is negligible and thus we have $P_{FA}=0\%$.

\vspace{0.1cm}
\noindent \textbf{Detecting suspension and injection attacks.}
% In the normal situation, authentication messages are transmitted continuously through the covert channel, and a message reception failure is mainly caused by occasional bit errors due to noise, and can be detected via the CRC check. 
% Let the probability of an erroneous frame in the normal situation be $\gamma$. 
% Hence, the probability of $K$ consecutive erroneous frames is $\gamma^K$, which decays exponentially as a function of $K$. 
% For example, with $\gamma=0.01$ and $K=3$, we have $\gamma^K = 10^{-6}$.
% In other words, it is very unlikely to have $K$ consecutive erroneous frames in the normal situation. 
As illustrated in Fig.~\ref{fig:example_of_iat_based_covert_channel_suspension}, when the suspension attack happens, the transmission of CAN messages is interrupted, which causes authentication message loss and thus message reception failures. 
Similarly, as shown in Fig.~\ref{fig:example_of_iat_based_covert_channel_injection}, the injection attack also interrupts the transmission of authentication messages, which causes either message loss or CRC errors. 
In this example, we use the 100-ms message with ID=0x139 from the EcoCAR as the attack message.
Since a CAN bus attack like the suspension or injection attack will need to last for a sufficient amount of time to cause enough damage to the CAN bus, it will cause more than $K$ consecutive message reception failures and thus can be detected by the TACAN-based detector with a detection probability of $100\%$. 

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=0cm 0.5cm 0cm 0cm,clip=true,width=1\textwidth]{Figures/example_of_iat_based_covert_channel_normal}
        \caption{Normal}
        \label{fig:example_of_iat_based_covert_channel_normal}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=0cm 0.5cm 0cm 0cm,clip=true,width=1\textwidth]{Figures/example_of_iat_based_covert_channel_suspension}
        \caption{Suspension attack}
        \label{fig:example_of_iat_based_covert_channel_suspension}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=0cm 0.5cm 0cm 0cm,clip=true,width=1\textwidth]{Figures/example_of_iat_based_covert_channel_injection}
        \caption{Injection attack}
        \label{fig:example_of_iat_based_covert_channel_injection}
    \end{subfigure}
    \caption{Illustration of the IAT-based covert channel in different situations using message 0x22A from the EcoCAR testbed: (a) normal, (b) under the suspension attack, and (c) under the injection attack.
    In both (b) and (c), the attack starts at around $t=10$ sec. 
    Under the suspension attack, the next message after the attack never arrives, and thus the next expected IAT (in dashed red) will keep increasing. 
    Both suspension and injection attacks will prevent the authentication message from being successfully received by the MN. 
    } 
    \label{fig:example_of_iat_based_covert_channel_under_attack}
\end{figure}


% \begin{figure}[t!]
% \centering
% \includegraphics[width=1\columnwidth]{./Figures/example_of_iat_based_covert_channel_under_attack}
% \caption{Example of the IAT-based covert channel in the normal situation (top), under the suspension attack (middle), and under the injection attack (bottom).
% Both suspension and injection attack will prevent the authentication message from being received by the MN. 
% }
% \label{fig:example_of_iat_based_covert_channel_under_attack}
% \end{figure}


\vspace{0.1cm}
\noindent \textbf{Detecting forgery attacks.}
In the forgery attack, the attacker has already compromised an in-vehicle ECU and transmits authentication messages, which can be successfully received by the MN (i.e., CRC check is passed). 
The attacker attempts to generate valid authentication messages which can be verified by the MN to evade the detection of TACAN. 

Since TACAN securely stores both master and session keys in the ECU's TPM to prevent being compromised by the adversary, the attacker has to forge a valid digest for each local counter value without the session key.
With a condensed digest of $M$ bits, the probability of a successful random forgery is $1/2^M$.
For example, when $M=8$, this probability is $1/2^8 \approx 0.4\%$.
In other words, the forgery attack will be detected with a probability of $99.6\%$ with $K=1$.
In general, the probability of $K$ consecutive message verification failures is $(1/2^M)^K$, which decreases as $K$ increases. 
%which is also the detection probability. 
Hence, to guarantee a desired detection probability for a given $K$, a suitable value of $M$ should be chosen.  
Repeated forgeries will be prevented due to the use of monotonic counters. 

\vspace{0.1cm}
\noindent \textbf{Detecting replay attacks.}
A replay attacker has infiltrated the CAN bus and attempts to replay previously transmitted authentication messages of the targeted ECU with the hope of passing the verification process at the MN.
It is easy to see that such attempts will be detected by TACAN with a probability of $100\%$ due to the use of monotonic counters. 

\vspace{0.1cm}
\noindent \textbf{Detecting masquerade attacks.}
As mentioned in Section~\ref{sec:adversary_model}, a masquerade attack (including the more sophisticated cloaking attack \cite{sagong2018cloaking}) requires in-vehicle ECUs to be weakly and/or fully compromised.
As a result, TACAN will force the attacker to perform a forgery or replay attack, not only for the compromised ECU itself, but also for the ECU the attacker attempts to masquerade as. 
Therefore, a masquerade attack will also be detected by TACAN. 

In summary, our proposed TACAN-based detector can identify attacks that interrupt the transmission of normal CAN messages (e.g., suspension and injection attacks), as well as attacks in which attackers fail to generate valid authentication messages (e.g., forgery, replay, and masquerade attacks) with a very high detection probability, while keeping the false alarm probability very low.


\subsection{Accuracy Loss}
\label{sec:eval:accuracy_loss}
In this section, we study the impact of LSB-based covert channel on the accuracy of sensor values. 
We first notice that with changes of a single bit ($L=1$), the accuracy loss has the same scale with the discretization error (resolution) of that sensor value. 
As $L$ increases, the overall throughput will increase (Section~\ref{sec:eval:throughput}), and the accuracy loss will also be larger. 
Hence, manufacturers will need to assess the impact of accuracy loss in CAN data on the functionality and safety, and trade off the accuracy loss against the throughput gain when deploying the LSB-based covert channel.
It is important to highlight that for periodic messages that cannot tolerate accuracy loss, manufacturers may deploy the IAT-based covert channel instead.


\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=-0.5cm 0.7cm 0cm 0cm,clip=true,width=.93\columnwidth]{./Figures/LSB_toyota_evaluation.eps}
        \caption{Wheel velocity}
        \label{fig:toyota_lsb_evaluation}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[trim=0cm 0.7cm 0cm 0cm,clip=true,width=.9\columnwidth]{./Figures/LSB_ecocar_evaluation.eps}
        \caption{Engine coolant temperature}
        \label{fig:ecocar_lsb_evaluation}
    \end{subfigure}
    \caption{Accuracy loss due to the LSB-based covert channel. (a) Wheel velocity in the Toyota dataset. (b) Engine coolant temperature in the EcoCAR dataset. We observe moderate accuracy loss in both cases. } 
    \label{fig:lsb_evaluation}
\end{figure}

In order to gain a better understanding of the accuracy loss of the LSB-based covert channel, we consider two CAN messages: 1) one that carries wheel velocity values from the Toyota dataset~\cite{toyota2010dataset} and 2) the one carries engine coolant temperature values that we identified through reverse engineering from the EcoCAR dataset~\cite{ecocar}.
In our experiments, we set $L$ to $1$ or $2$ and quantify the accuracy loss in terms of the maximum error, i.e., the maximum deviation from the original values (which are considered as ground truth). 
Note that we intentionally keep $L \leq 2$ in order to avoid significant distortions to the underlying sensor values or jeopardize the functionality of the receiving ECU.

As illustrated in Fig.~\ref{fig:toyota_lsb_evaluation} and highlighted in the magnified box, the maximum error introduced to wheel velocity is $0.01$ km/h for $L=1$ and $0.03$ km/h for $L = 2$, which is considered as insignificant. 
As for the engine coolant temperature in  Fig.~\ref{fig:ecocar_lsb_evaluation}, the maximum error is $1$ $^{\circ}C$ for $L = 1$ and $3$ $^{\circ}C$ for $L = 2$, which are still moderate.
As compared to the median value of $58$ $^{\circ}C$, the errors of $1$ $^{\circ}C$ and $3$ $^{\circ}C$ translate into $1.7\%$ and $5.2\%$ deviations, respectively.

==> TACAN Extension (arXiv)/Sections/intro.tex <==
\IEEEraisesectionheading{\section{Introduction}}
\label{sec:introduction}

\IEEEPARstart{N}{owadays}, the technological evolution enables an increasingly more invasive interconnection between automobiles and digital devices.
%Thanks to the network connectivity, the 
Automotive manufacturers have developed a variety of innovative features such as the smart transportation data assistants by leveraging network connectivity such as the vehicle-to-vehicle communication.
%These features increase comfort for the costumers offering useful services, but on the other hand, they open new surfaces of cyber-physical vulnerabilities.
While these features greatly improve the customer experience, Electronic Control Units (ECUs) that are externally accessible provide an entry point for an adversary to infiltrate the originally isolated in-vehicle communication network, notably the Controller Area Network (CAN) \cite{ISO2015CAN,bosch1991CAN}.
%Electronic Control Units (ECUs) that are externally accessible may expose other in-vehicle ECUs on the same Controller Area Network (CAN) bus to the outside world, thus opening up new attack surfaces for possible exploits.
%\rev{Due to the coupling between the cyber and physical components of an automobile, a compromised ECU can also potentially cause potential  }
%In this scenario, modern cars are no longer engineering systems where the electronics plays a secondary role: even low-end cars have several Electronic Control Units (ECUs) embedded. ECUs execute millions of lines of software code, controlling everything from the brakes to the radios.
%Looking ahead to the near future, autonomous vehicles will become part of our lives and it is straightforward to consider potential issues to the new automotive generation security with the related threats for human safety.
%\giuseppe{Even though the innovation is relevant for the automotive industry, the insecure Controller Area Network (CAN) bus continues to be used as communication medium for the in-vehicle networks~\cite{ISO2015CAN,bosch1991CAN}.
%The Controller Area Network (CAN) enables communication among Electronic Control Units (ECUs) for closed in-vehicle networks~\cite{ISO2015CAN,bosch1991CAN}.
%\rev{Due to the widespread use of the legacy CAN bus, securing the CAN bus is of paramount importance for the functionality and safety of today's vehicles and future's autonomous cars~\cite{bojarski2016end,wyglinski2013security}.}
%Therefore, the development of novel methodologies to secure the CAN bus is of paramount importance for the functionality and safety of today's vehicles and future's autonomous cars~\cite{bojarski2016end,wyglinski2013security}.
Since the CAN bus is a broadcast medium without authentication, a compromised ECU can masquerade as any targeted ECU by transmitting messages with the forged message ID (masquerade attack~\cite{checkoway2011comprehensive}).
Modern externally accessible ECUs
with additional connectivity interfaces such as cellular, Wi-Fi or Bluetooth %(e.g., advanced car radios) 
disrupt the closed in-vehicle network assumption.
Consequently, the CAN bus is vulnerable to cyber attacks, such as disabled brakes~\cite{checkoway2011comprehensive} and remotely controlled steering~\cite{tesla2016remote}.
%Recent studies have shown that through compromised ECUs, attackers are able to disable breaks \cite{checkoway2011comprehensive}, remotely control steering \cite{tesla2016remote}, or disable vehicles on a highway \cite{wired2015remote}. 
Despite of the well-known security vulnerabilities of the CAN bus, its widespread use imposes an urgent need for security solutions that  guarantee the functionality and safety of today's automobiles and future's autonomous cars~\cite{bojarski2016end,wyglinski2013security}.

The use of cryptographic primitives, such as message authentication, represents one possible way to defend against CAN bus attacks (notably the masquerade attack).
However, due to the low throughput and tight bit budget of the CAN protocol, it is challenging to deploy cryptographic schemes in practice and current solutions, such as~\cite{herrewege2011canauth,hazem2012lcap,kurachi2014cacan,radu2016leia}, would require protocol modifications or introduce traffic overheads.
%introduce protocol overheads or increase the bus load. 
An alternative is to deploy anomaly-based Intrusion Detection Systems (IDSs) without modifying the CAN protocol~\cite{cho2016finger,muter2011entropy,cho2017viden,choi2018voltageids}, including timing-based and voltage-based IDSs.
%one leveraging the timing of CAN messages ad the other one exploiting the voltage of CAN signals on the bus. 
The timing-based IDS in~\cite{cho2016finger} exploits CAN message periodicity to estimate clock skew as a unique fingerprint to detect masquerade attacks. 
Nevertheless, it was later shown to be ineffective against the cloaking attack that modifies the inter-transmission time to emulate the clock skew of the targeted ECU~\cite{sagong2018cloaking,ying2018shape}. 
The voltage-based IDSs~\cite{murvay2014source,cho2017viden,choi2018voltageids,kneib2018scission} attempt to %can effectively 
%choi2018identifying
fingerprint the attacker through voltage signal characteristics. 
However, if the attacker uses IDs that the compromised ECU is allowed to use under normal conditions, the attack will not be detected.

%it cannot detect a compromised ECU (a persistent attacker) before a masquerade attack is launched. 

\begin{figure}[t!]
\centering
\includegraphics[width=1\columnwidth]{./Figures/main_idea}
%\vspace{-0.6cm}
\caption{Illustration of TACAN. Legitimate ECUs transmit unique authentication messages that are embedded into the timing and LSBs of normal CAN messages (e.g., A1, B2, and C3) using the proposed covert channel methodologies. 
The Monitor Node authenticates transmitting ECUs by verifying the received authentication messages. If the compromised ECUs cannot generate valid authentication messages, then the attack will be detected by the Monitor Node.}
\label{fig:main_idea}
%\vspace{-0.2cm}
\end{figure}

In this work, we present TACAN, a novel security framework that allows a centralized, trusted \textit{Monitor Node} (MN) to verify the authenticity of a transmitting ECU and detect CAN bus anomalies. Fig.~\ref{fig:main_idea} highlights the main idea of our TACAN framework.
%develop a transmitter authentication scheme through covert channels to detect ongoing attacks and persistent attackers without modifying the CAN protocol or increasing the bus load. 
%each ECU to transmit unique authentication sequences over the CAN bus through covert channels without protocol modifications or overheads.
%Inspired by the physical-layer transmitter authentication techniques in wireless communication \cite{kumar2014blind,liu2010authenticating,yang2012enforcing},
In TACAN, a master key is shared between an ECU and the MN for generating shared session keys. 
Consistently with \cite{hazem2012lcap,radu2016leia, herrewege2011canauth}, we assume that the keys are stored in the tamper-resistant memory of a security module such as the Trusted Platform Module (TPM) \cite{TPMautomotive}. %that can be used to secure the ECUs~\cite{TPMautomotive}.
%
%
%both of which are stored in \giuseppe{a Trusted Platform Module (TPM)\footnote{\giuseppe{Since more ECUs are being added and there usually exist multiple CAN buses in a vehicle, coordinating or gateway ECUs are expected to be high-grade and trusted. We assume TPMs as tamper-resistant memories and can be used to secure the ECUs~\cite{TPMautomotive}.}}}.
%which creates a need for TPM.
%A real-world example of TPM is provided in~\cite{infineon2011tpm}.}.}
%TACAN deploys a pre-shared between each ECU and the MN in the tamper-proof storage for generating shared session keys.
%
%
The ECU embeds unique authentication messages into CAN messages and continuously transmits them through covert channels, which can be received and verified by the MN.
%Since 

Therefore, if the attacker has no access to the TPM of the targeted ECU, %when it compromises an ECU or masquerades as other ECUs, 
it cannot use the compromised ECU or external device to generate valid authentication messages, thus causing verification failures and triggering the alarm at the MN side.
Moreover, CAN bus attacks, such as the suspension and injection attacks, that interrupt the transmission of normal CAN messages with embedded authentication messages will cause continuous authentication message loss or reception failures, and therefore they will be detected by TACAN.
The main benefits of using covert channels for TACAN are that they do not introduce protocol modifications or traffic overheads (i.e., extra bits or messages).
In addition, by requiring ECUs to transmit authentication messages much less frequently than per-message authentication schemes, TACAN can significantly reduce the computational burden of the resource-constrained ECUs.


%Compared to existing per-message authentication schemes~\cite{herrewege2011canauth,hazem2012lcap,kurachi2014cacan,radu2016leia}, TACAN requires considerably less computational resources at both transmitter and receiver, and does not introduce protocol modifications or overheads thanks to covert channels.

\vspace{0.1cm}
\noindent \textbf{Contributions: }
In this paper, we make the following contributions: 
\begin{itemize}
    \item We identify and exploit covert channels to facilitate ECU authentication on the CAN bus. 
    Hence, covert channels are used for security instead of malicious communication.
    
    %We introduce the notion of transmitter authentication to CAN bus security and turn the originally malicious concept of covert channels into an application that enables the communication between the ECU and the MN.
    
    \item We propose TACAN and three novel covert channels for authentication message transmission: 1) the IAT (Inter-Arrival Time)-based covert channel that modifies the inter-transmission times (ITTs) of normal CAN messages to affect the IATs observed by the MN;
    2) the LSB (Least Significant Bit)-based covert channel that hides the authentication bits in the LSBs of the data payload of normal CAN messages; 
    3) an hybrid covert channel that combines the first two covert channels.
    
    \item For the IAT-based covert channel, we analyze and model the bit error probability as a function of covert channel parameters. We also study its impact on the CAN bus schedulability in terms of the worst-case response time.

    \item We validate TACAN and the covert channels on the UW EcoCAR~\cite{ecocar}. 
    We also conduct extensive experiments to evaluate the performance of TACAN using the EcoCAR testbed as well as the publicly available Toyota dataset~\cite{toyota2010dataset}.
    Our results show that with a properly configured IAT-based covert channel, the experimental bit error probabilities are within 0.3\%. 
    As for the LSB-based covert channel, its bit error probability is equal to that of a typical CAN bus, which is $3.1\times 10^{-7}$\%. 
    The hybrid covert channel generally leads to higher channel and authentication throughput.
    We also show that our TACAN-based detector can detect CAN bus attacks with a very high detection probability, while keeping the false alarm probability less than 0.33\% by setting the detection threshold to $2$ or higher.
    
    
    %Our results show that the bit error ratios are within $0.1\%$ and $0.42\%$ for the IAT-based and offset-based covert channels, respectively. The bit error ratio of the LSB-based covert channel is equal to $3.1\times 10^{-7}$\%, which is the bit error ratio of a typical CAN bus.
\end{itemize}

\noindent \textbf{Organization.}
The remainder of this paper is organized as follows.
Section~\ref{sec:related_work} reviews the related work.
Section~\ref{sec:system_and_adversary_model} presents our system and adversary models.
Section~\ref{sec:proposed_scheme} presents TACAN. 
%A security discussion of TACAN is provided in Section~\ref{sec:security_analysis}. 
Section~\ref{sec:evaluation} presents experimental evaluation.
Section~\ref{sec:conclusion} concludes this paper. 

==> TACAN Extension (arXiv)/Sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Recent experimental studies have demonstrated that an attacker is able to infiltrate in-vehicle ECUs physically or remotely and mount cyber attacks that would cause potentially life-threatening consequences by disabling brakes or overriding steering~\cite{miller2015remote,checkoway2011comprehensive}.
One way to secure the CAN bus is to deploy anomaly-based IDSs based on traffic analysis (e.g., timing/frequency~\cite{hoppe2008security}), % miller2013adventure
%and contents~\cite{kang2016intrusion})
entropy~\cite{muter2011entropy}, or physical invariants such as clock skew~\cite{cho2016finger} and voltage signal characteristics~\cite{murvay2014source,cho2017viden,choi2018voltageids,kneib2018scission}. 
For clock skew-based IDSs, it has been shown in \cite{sagong2018cloaking,ying2018shape} that the adversary can effectively manipulate the timing of transmitted messages to emulate the clock skew of the targeted ECU and evade the detection.
While voltage-based IDSs are effective against ongoing masquerade attackers, they cannot detect a compromised ECU before attacks are launched (e.g., a stealthy attacker may not launch the attack until the car is in drive mode). 
In addition, it has been recently shown in \cite{sagong2018exploring} that the extra wires required by voltage-based IDSs may introduce new attack surfaces.

Researchers have also proposed to add cryptographic primitives such as Message Authentication Code (MAC) to the CAN bus, including CANAuth~\cite{herrewege2011canauth}, LCAP~\cite{hazem2012lcap}, CaCAN~\cite{kurachi2014cacan}, and LeiA~\cite{radu2016leia}. 
Nevertheless, the deployment of the above schemes faces several practical challenges. First, the CAN protocol has a tight bit budget for each CAN frame (up to 8 bytes for payload) and a low bus speed (typically 500 kbps). 
As a result, authentication information will have to consume space in the CAN message such as the ID or data field or introduce additional CAN messages, which leads to traffic overheads or an increase in the bus load~\cite{hazem2012lcap,kurachi2014cacan,radu2016leia}.
Second, it is also computationally expensive for resource-constrained ECUs to perform cryptographic calculations for each message.
In this work, we focus on transmitter authentication by having each ECU transmit unique authentication messages as its digital fingerprint.
%focus on transmitter authentication rather than per-message authentication to avoid such traffic overheads. 
The main novelty of this work is the use of covert channels, a well-known malicious technique that is converted into defensive applications for authentication purposes.
By leveraging covert channels as out-of-band channels, our scheme can avoid traffic overheads without requiring protocol modifications.
%or introduce extra bits or CAN messages.

In literature, a covert channel refers to a type of cyber-attack that maliciously transfers information between two possibly malicious entities by exploiting the communication channels that are not intended for information transfer. 
It has been widely studied in computer network protocols \cite{zander2007survey}.
Broadly speaking, there are two categories of covert channels: timing-based and storage-based. 
In timing-based covert channels, only the timing of events or traffic is modified to transfer information but the data contents remain intact.
The storage-based covert channels hide data in a shared resource (e.g., a storage location). % that is not designed for transferring data. 
%, e.g., by exploiting reserved or used fields in the data packet or concealing data in the payload \shaun{(Do we want to modify this?)}.
%Compared to steganography techniques that require some form of contents as cover, the covert channels exploit network protocols as carrier~\cite{zander2007survey}.

Recently, researchers start exploring covert channels in the context of embedded networks.
In~\cite{taylor2017enhancing}, Taylor \textit{et al.} discussed the use of covert channels for integrity check for the Modbus/TCP protocol used by industrial control system applications.
In \cite{groza2018incanta}, Groza \textit{et al.} proposed a time-covert authentication scheme for the CAN protocol, which uses fine-grained timing control to embed authentication information in clock skews.
However, timing control in the order of tens of nanoseconds is challenging in practice, and the proposed scheme is very sensitive to message priority and the traffic. 
In addition, since the clock skew needs to be estimated from arrival times of many CAN messages, it seems to contradict with the proposed scheme that performs authentication for each CAN message.
%\giuseppe{Groza \textit{et al.} present in~\cite{groza2018incanta} a timing-based covert channel authentication technique for the CAN bus. This authentication scheme, namely INCANTA, exploits clock skews for authentication and intrusion detection aims on the in-vehicle networks. Compared to INCANTA, our schemes are more practical, flexible, and with a larger throughput thanks to the definition of the LSB-based and Hybrid implementations.}
%To the best of our knowledge, this is the first paper that explores \giuseppe{different techniques of} covert channels for automotive CAN buses.

In this paper, we develop three practical covert channels for transmitter authentication on the legacy CAN bus, based on the periodicity of CAN messages and bit presentation of floating sensor values. We also evaluate the proposed covert channels using CAN traffic data collected from real vehicles.

==> TACAN Extension (arXiv)/Sections/security_analysis.tex <==
\section{Security Discussion \shaun{(To be updated)}}
\label{sec:security_analysis}
%In this section, we provide a security discussion of TACAN.
Compared to the existing message authentication schemes \cite{herrewege2011canauth,hazem2012lcap,kurachi2014cacan,radu2016leia} that attempt to verify the authenticity of each message, TACAN extracts and verifies authentication message embedded in the timing or LSBs of normal messages to authenticate the transmitting ECU and also serves the purpose of intrusion detection.
%While TACAN cannot detect spoofed messages (since it does not examine the message content), 
Hence, TACAN can detect attacks that interrupt the transmission of normal CAN messages (e.g., suspension, injection, and DoS attacks), as well as attacks in which attackers fail to generate valid authentication messages (e.g., forgery, replay, and masquerade attacks). 
The above security properties provided by TACAN are independent of the CAN protocol and the contents of CAN messages.
%The main advantage of TACAN is that it does not require protocol modifications or introduce traffic overheads (i.e., no extra bits or messages).
%Moreover, since ECUs are resource-constrained and authentication message generation can be computationally expensive, TACAN can significantly reduce the computational burden on ECUs by requiring them to transmit authentication messages much less frequently than per-message authentication schemes.
%In the rest of this section, we will discuss how TACAN is able to detect the aforementioned attacks in more detail.
%\revv{In the rest of this section, we will discuss the security features of TACAN and how it detects forgery, replay, and masquerade attacks in more detail.}

%In particular, we discuss how TACAN is able to detect forgery, replay, and masquerade attacks.

\vspace{0.1cm}
\noindent \textbf{Security Features.}
We summarize a list of features provided by TACAN as follows: 1) TACAN securely stores both master and session keys in the ECU's TPM to prevent being compromised by the adversary, 2) TACAN employs monotonic counters for generating session keys and authentication messages for each ECU, and 3) TACAN requires each ECU to continuously transmit unique authentication messages to enable real-time transmitter authentication.

Note that due to the third feature, if the attacker compromises an in-vehicle ECU but does not attempt to deceive TACAN (i.e., stop generating authentication messages), it will interrupt the continuous transmission of authentication messages and thus will be detected immediately.
In addition, since basic attacks like suspension, injection, and DoS attacks can be easily detected, we focus on more sophisticated attacks in the rest of this section that actively attempt to evade TACAN, including the forgery attack, the replay attack, and the masquerade attack.

\vspace{0.1cm}
\noindent \textbf{Detecting Forgery Attacks.}
In the forgery attack, the adversary has already compromised an in-vehicle ECU that is protected by TACAN and attempts to generate valid authentication messages that can be verified by the MN in order to evade the detection of TACAN. 
Since our adversary model (Section~\ref{sec:adversary_model}) assumes that the attacker has no access to the TPM of the compromised ECU, the attacker has to forge a valid digest for each local counter value without the session key.
With a condensed digest of $M$ bits, the probability of a successful forgery is $1/2^M$.
For example, when $M=8$, this probability is $1/2^8 \approx 0.4\%$.
Repeated forgeries will be prevented due to the use of monotonic counters. 

\vspace{0.1cm}
\noindent \textbf{Detecting Replay Attacks.}
A replay attacker has infiltrated the CAN bus and attempts to replay previously transmitted authentication messages of the targeted ECU with the hope of passing the verification process at the MN.
It is easy to see that such attempts will be detected by TACAN due to the use of monotonic counters. 

% \vspace{0.1cm}
% \noindent \textbf{Detecting Compromised ECUs.}
% Our adversary model (Section~\ref{sec:adversary_model}) assumes that the attacker has no access to both the master and session keys stored in the TPM of the compromised ECU.
% In order to deceive TACAN, the attacker has to forge a valid digest for each local counter value without the session key.
% With a condensed digest of $M$ bits, the probability of a successful forgery is $1/2^M$.
% For example, when $M=8$, this probability is $1/2^8 \approx 0.4\%$.
% Repeated forgeries and replay attacks will not work because the local counter is incremented monotonically. 
% Therefore, a compromised ECU will be detected by TACAN with very high probability.

% \vspace{0.1cm}
% \noindent \textbf{Detecting Suspension Attacks.}
% Since a suspension attack requires a compromised in-vehicle ECU, this attack will be readily detected by TACAN, according to our previous discussion.
% Moreover, suspending a CAN message that carries authentication messages between the ECU and the MN will also interrupt the underlying covert channel, which can be detected by the MN. 

% \vspace{0.1cm}
% \noindent \textbf{Detecting Fabrication Attacks.}
% If the fabrication attack requires compromising an in-vehicle ECU, it will be detected by TACAN; otherwise, it needs to be launched from an external device.
% There are two cases of message fabrication.
% In the first case, non-existent message IDs are used (e.g., using 0x00 for launching the DoS attack). 
% Such attacks will not be detected directly by TACAN. 
% In the second case, existing message IDs are used.
% The attack will be detected by TACAN, if the targeted message is used to deploy the covert channel. 
% In either case, if the attacker introduces abnormal CAN traffic that interrupts the deployed covert channels, TACAN will raise an alarm. 
% Nevertheless, existing IDSs such as \cite{hoppe2008security,miller2013adventure} can always be deployed in conjunction with TACAN to enhance the CAN bus security.

\vspace{0.1cm}
\noindent \textbf{Detecting Masquerade Attacks.}
As mentioned in Section~\ref{sec:adversary_model}, a masquerade attack (including the more sophisticated cloaking attack \cite{sagong2018cloaking}) requires in-vehicle ECUs to be weakly and/or fully compromised.
As a result, TACAN will force the attacker to perform a forgery or replay attack, not only for the compromised ECU itself, but also for the ECU the attacker attempts to masquerade as. 
Therefore, a masquerade attack will be detected by TACAN. 
% , which can be detected by the TACAN before the onset of the attack.
% In addition, since a masquerading attacker has no access to the keys stored in the TPM of the targeted ECU, it will not be able to forge valid authentication messages that can pass the verification process at the MN. 

% \shaun{As mentioned in Section~\ref{sec:adversary_model}, a stealthy masquerade attack would require in-vehicle ECUs to be weakly and/or fully compromised, which can be detected by the MN before the onset of the attack.
% In general, when a compromised ECU or an external device attempts to masquerade as another ECU (by simply faking the message ID), the authentication message transmission of the targeted ECU may be interrupted, thus causing the MN to raise an alarm.
% Moreover, since the adversary has no access to the keys stored in the TPM of the targeted ECU, it will not be able to generate valid authentication sequences anyway. }

%In order to launch stealthy masquerade attacks, the attacker will need to compromise two ECUs -- one is weakly compromised and the other one is fully compromised \cite{lin2012cyber,cho2016finger}. 
%During the attack, the attacker suspends the weakly compromised ECU A from transmitting certain messages and uses the fully compromised ECU B to inject messages claiming to originate from ECU A. 
%As we can see, since the attacker has no access to the ECU A's private key, it will not be able to generate valid authentication messages for ECU A, and blind forgery can hardly succeed as discussed in the previous section.
%The premise that two ECUs need to be compromised already allows the MN to identify compromised ECUs and prevent masquerade attacks from happening.

\vspace{0.1cm}
% \noindent \textbf{Robustness Against Replay Attacks.}
% While the attacker is able to observe the current and all previous authentication messages transmitted by the targeted ECU, it is computationally unfeasible to launch replay attacks due to the built-in local counter in authentication messages. 
% Whenever the local counter overflows, the global counter will be incremented by one and a new session key will be generated. 
% Since each session key should be used only once for the lifetime of the vehicle, the same local counter value will not be signed by the same session key twice, which makes replay attacks extremely difficult, if not impossible. 

%\vspace{0.1cm}
% \noindent \textbf{Robustness Against Other Attacks.}
% In practice, it is possible to launch other attacks such as the suspension, fabrication, and DoS attacks.
% \shaun{If an attack (e.g., suspension attack) requires an in-vehicle ECU to be compromised, it can be readily detected by TACAN.}
% \shaun{On the one hand, if TACAN is deployed for all messages and the attacker injects messages with existing IDs, the resulting authentication message for the spoofed CAN message will fail the verification process at the MN and an alarm will be triggered.
% On the other hand, message injection using non-existence IDs can be easily detected, even without TACAN.}
% In practice, existing IDSs such as \cite{hoppe2008security,miller2013adventure} can also be deployed in conjunction with TACAN to enhance the CAN bus security.


==> TACAN Extension (arXiv)/Sections/system_model.tex <==
\section{System and Adversary Models}
\label{sec:system_and_adversary_model}
In this section, we present the system model (Section~\ref{sec:system_model}) and the adversary model (Section~\ref{sec:adversary_model}) for the CAN bus.
A list of frequently used notations is provided in Table~\ref{table:notation}.

\begin{table}[t!]
	%\footnotesize
	\centering
	\caption{Frequently used notations.
	%\shaun{SK generation counter}
	%\giuseppe{``epoch'' or ``generation'' instead of ``global''. By the way ``epoch'' is used in the LeiA paper, so better to use generation with ``G'' as symbol. }
	}
	%\vspace{-0.1cm}
	\begin{tabular}{|c|l|}
		\hline
		\textbf{Notation} & \textbf{Description} \\
		\hline
		$MK^{(k)}$ & Master key (MK)  for message ID $k$ \\ \hline
		$SK^{(k)}$ & Session key (SK) for message ID $k$ \\ \hline
		$C_{s}^{(k)}$ & Session key counter for message ID $k$ \\ \hline
		$C_{m}^{(k)}$ & Authentication message counter for message ID $k$\\ \hline
		$T$ & CAN message period (sec)\\ \hline
		$S$ & Clock skew (ppm) \\ \hline
		$t_i$ & Transmit time of the $i$-the CAN message \\ \hline
		$a_i$ & Arrival time of the $i$-the CAN message \\ \hline
		$\eta_i$ & Noise in the arrival time of the $i$-the CAN message \\ \hline
		\multirow{ 2}{*}{$\Delta t_i$} & Inter-transmission time (ITT) between the $(i-1)$-th \\ & and the $i$-th messages \\ \hline
		\multirow{ 2}{*}{$\Delta a_i$} & Inter-arrival time (IAT) between the $(i-1)$-th \\& and the $i$-th messages \\ \hline
		$\Delta \bar{a}[i]$ & The $i$-th sample of averaged IATs\\ \hline 
		$\delta$ & Deviation (added to ITTs at the transmitter side) \\ \hline
		$L$ & Window length or number of least significant bits \\ \hline
		$\mu, \sigma$ & Mean and standard deviation of IATs \\ \hline 
		
	\end{tabular}
	
	\label{table:notation}
	\normalsize
	%\vspace{-0.1cm}
\end{table}

\subsection{System Model}
\label{sec:system_model}

\noindent \textbf{CAN bus.}
The CAN bus is a broadcast medium that allows all connected ECUs to communicate with each other and observe all CAN message transmissions.
As shown in Fig.~\ref{fig:can_frame_structure}, each CAN frame or message has a set of predefined fields, including the Start of Frame (SOF) field, the Arbitration field (including a 11-bit message ID for the base frame format or a 29-bit message ID for the extended frame format), the Control field, the Data field (up to 8 bytes), the Cyclic Redundancy Check (CRC) field, the Acknowlegement (ACK) field, and the End of Frame (EOF) field.

\begin{figure}[ht!]
\centering
\includegraphics[width=1\columnwidth]{./Figures/can_frame_structure}
\caption{Illustration of CAN frame structure.}
\label{fig:can_frame_structure}
%\vspace{-0.3cm}
\end{figure}

When two (or more) ECUs attempt to transmit messages at the same time, a procedure based on priority (a smaller message ID indicates a higher priority) called arbitration is used to determine the winner. 
Besides, CAN messages do not have transmit timestamps and do not support encryption or authentication. 

\vspace{0.1cm}
\noindent \textbf{Clock skew.} 
On automotive CAN buses, the majority of CAN messages are  transmitted periodically as per ECUs' local clocks\footnote{In the UW EcoCAR (Chevrolet Camaro 2016) \cite{ecocar}, all of the 89 messages with distinct IDs are periodic with periods ranging from 10 ms to 5 sec. In the Toyota Camry 2010 \cite{toyota2010dataset}, 39 of 43 messages can be considered periodic. In the Dodge Ram Pickup 2010 in \cite{cho2016finger}, all of the 55 distinct messages are periodic. While CAN message periodicity depends on the manufacturer and the model, the above examples suggest that periodic CAN messages are very common and even dominant on the CAN bus of commercial automobiles.}, and there is no clock synchronization in CAN.
Hence, the frequencies of local clocks are different, as captured by the notion of clock skew -- a physical property caused by variations in the clock's hardware crystal. 

Let $\mathcal{C}_A(t)$ be the time reported by clock $A$ and $\mathcal{C}_{true}(t)=t$ be the true time. 
According to the Network Time Protocol (NTP)~\cite{mills1992NTP}, the clock offset of clock A is defined as $O_A(t)=\mathcal{C}_A(t)-\mathcal{C}_{true}(t)$, 
% \begin{equation}
%     O_A(t)=C_A(t)-C_{true}(t), \label{eq:clock_offset}
% \end{equation}
and the clock skew is the first derivative of clock offset, i.e., $S_A(t)=O'_A(t)=\mathcal{C}'_A(t)-1$, which is measured in microseconds per second ($\mu$s/s) or parts per million (ppm).
In the absence of a true clock, the relative clock offset and relative clock skew can be defined with respect to a reference clock.
Throughout this paper, we consider the receiving ECU's clock as the reference clock. Hence, we refer to the relative clock offset and the relative clock skew as clock offset and clock skew, respectively.

\vspace{0.1cm}
\noindent \textbf{Timing model.}
As shown in Fig.~\ref{fig:timing_model}, we let $t_i$ be the transmit time of message $i$ (assuming $t_0=0$) and $\Delta t_i = t_i - t_{i-1}$ be the inter-transmission time (ITT) according to the transmitter's clock.
If messages are periodically transmitted every $T$ seconds, we have $\Delta t_i=T$ and $t_i=iT$. 
In the ideal case where the transmitter's clock is synchronized with the receiver's clock, we have $t'_i=t_i$, where $t'_i$ is the transmit time according to the receiver's clock. 
Nevertheless, in practice, there exists a clock skew in the transmitter's clock relative to the reference clock, which introduces an offset $O_i$ between the two clocks. 
Hence, the actual transmit time is $t'_i = t_i - O_i$ according to the reference clock. 

While the clock skew may be slowly varying due to factors including the temperature, it is almost constant over a short duration.
Given a clock skew $S$, the relationship between the elapsed time $t_i$ in the transmitter's clock and the elapsed time $t'_i$ in the receiver's clock is $S = (t_i - t'_i)/t'_i$.
Hence, we have $t_i' = t_i/(1+S)$, and $O_i = t_i - t_i' = \frac{S}{1+S} t_i$.
To capture random jitters, we assume $O_i = \frac{S}{1+S} t_i + \epsilon_i$, 
% \begin{equation*}
%     O_i = \frac{S}{1+S} t_i + \epsilon_i,
% \end{equation*}
where $\epsilon_i$'s are i.i.d. zero-mean random variables.

\begin{figure}[t!]
\centering
\includegraphics[trim=0cm 0.7cm 0cm 0cm, clip=true, width=1\columnwidth]{./Figures/timing_model}
\caption{Illustration of our timing model. 
Due to the clock skew of the transmitter's clock, the actual transmit time of message $i$ is $t_i'=t_i-O_i$ as per the receiver's clock, where $O_i$ is the accumulated clock offset up to message $i$. 
}
\label{fig:timing_model}
\end{figure}

After a random network delay of $d_i$ (due to message transmission, propagation, arbitration, and reception) and the zero-mean quantization noise $q_i$~\cite{zander2008measurement}, the arrival time of message $i$ is
\begin{align}
    a_i &= t_i - O_i + d_i + q_i \nonumber\\
    &=t_i - \frac{S}{1+S} t_i  + \eta_i =\frac{1}{1+S}t_i + \eta_i, \label{eq:arrival_timestamp}
\end{align}
where $\eta_i = -\epsilon_i + d_i + q_i$ is the total noise in the arrival timestamp. 
Since periodic CAN messages have the same message ID and  data length over time, it is reasonable to assume constant-mean network delays, i.e., $\mathbb{E}[d_i] = d$. 
%Hence, $\eta_i$'s can be modeled as i.i.d. Gaussian random variables with $\eta_i \sim N(d, \sigma^2_\eta)$. 
Hence, $\eta_i$'s can be modeled as i.i.d. random variables with a mean of $d$ and a variance of $\sigma_\eta^2$. 

Denote the inter-arrival time (IAT) between messages $(i-1)$ and $i$ as $\Delta a_i$, which is given by
\begin{equation}
    \Delta a_i = a_i - a_{i-1} = \frac{1}{1+S} \Delta t_i + n_i, \label{eq:inter_arrival_time}
\end{equation}
where $n_i=\eta_i - \eta_{i-1}$ is the noise term.
For messages that are transmitted every $T$ seconds, we have $\Delta t_i = T$. 
Hence, the IATs have a mean of
\begin{equation}
    \mu \triangleq \mathbb{E}[\Delta a_i] = \frac{T}{1+S} \label{eq:IAT_mean}
\end{equation}
and a variance of 
\begin{equation}
    \sigma^2 \triangleq \text{Var}[\Delta a_i] = 2\sigma_\eta^2. \label{eq:noise_variance}
\end{equation}
When the clock skew is small (in the order of 100s of ppm), the impact of clock skew is negligible, and we have $\mu \approx T$. 


\subsection{Adversary Model}
\label{sec:adversary_model}
We consider an adversary who attempts to infiltrate the CAN bus and launch stealthy attacks without being detected.
We assume that the adversary can passively monitor the CAN bus and observe all ongoing CAN transmissions. 
It has full knowledge of the deployed covert channels and thus can observe all authentication messages that are being transmitted.
In practice, there are usually two ways of gaining unauthorized access to the CAN bus: 1) compromise an in-vehicle ECU physically or remotely~\cite{checkoway2011comprehensive}, or 2) connect external device (a malicious ECU) to the CAN bus~\cite{koscher2010experimental}.
We assume that the adversary has no access to the keys stored in the TPM of the compromised and other legitimate ECUs.
%Nevertheless, we assume that the adversary does not have access to the TPM, even if it is able to fully compromises an ECU (e.g., reprogram the firmware).

The adversary can use the compromised or malicious ECU to perform three representative attacks: 1) suspension attack, 2) injection attack, and 3) masquerade attack, as considered in~\cite{lin2012cyber,cho2016finger,sagong2018cloaking}.
As illustrated in Fig.~\ref{fig:attack_suspension}, a suspension attacker prevents the compromised ECU from transmitting certain messages, whereas an injection attacker fabricates and injects CAN messages of arbitrary choices of message ID, content, and timing, as sketched in Fig.~\ref{fig:attack_fabrication}.
Injection attacks can lead to more sophisticated attacks such as the DoS %Denial-of-Service (DoS) 
attack~\cite{hoppe2008security} and the bus-off attack~\cite{cho2016error}. 
%, in which the attacker exploits the arbitration process and constantly injects higher priority messages (with lower IDs) to prevent legitimate messages from being transmitted. 
In the masquerade attack, the adversary will need to compromise two ECUs -- one is weakly compromised and acts as the weak attacker who can only launch suspension attacks, whereas the other one is fully compromised and acts as the strong attacker who can launch both suspension and injection attacks. 
In the example in Fig.~\ref{fig:attack_masquerade}, the adversary suspends the weakly compromised $\text{ECU}_2$ from transmitting messages with ID=0x22 and uses the fully compromised $\text{ECU}_1$ to inject messages with ID=0x22 claiming to originate from $\text{ECU}_2$. 
Compared to the suspension and injection attacks, the masquerade attack is stealthier and thus more difficult to detect. 

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[width=\textwidth]{Figures/attack_suspension}
        %\vspace{-0.5cm}
        \caption{Suspension attack}
        \label{fig:attack_suspension}
    \end{subfigure}
    
    \vspace{0.2cm}
    
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[width=\textwidth]{Figures/attack_fabrication}
        %\vspace{-0.5cm}
        \caption{Injection attack}
        \label{fig:attack_fabrication}
    \end{subfigure}
    
    \vspace{0.2cm}
    
    \begin{subfigure}[b]{1\columnwidth}
        \includegraphics[width=\textwidth]{Figures/attack_masquerade}
        %\vspace{-0.5cm}
        \caption{Masquerade attack}
        \label{fig:attack_masquerade}
    \end{subfigure}
    
    %\vspace{-0.2cm}
    \caption{Three representative attacks on the CAN bus. (a) In the suspension attack, a legitimate message is prevented from being transmitted. 
    (b) In the fabrication attack, the adversary can use the compromised ECU to inject arbitrary CAN messages. 
    (c) In the masquerade attack, the adversary stops $\text{ECU}_2$ from transmitting messages with ID=0x22 and uses $\text{ECU}_1$ to transmit messages with ID=0x22.
    }
    \label{fig:attack_model}
    %\vspace{-0.3cm}
\end{figure}

==> TACAN Extension (arXiv)/Sections/tacan.tex <==
\section{TACAN}
\label{sec:proposed_scheme}
In this section, we present the architecture (Section~\ref{sec:tacan_architecture}) and the transmitter authentication protocol of TACAN (Section~\ref{sec:transmission_authentication_protocol}).
We then present three covert channels for transmitting authentication messages: 
1) IAT-based (Section~\ref{sec:IAT_based_covert_channel}), 2) LSB-based (Section~\ref{sec:lsb_based}), and 3) hybrid  (Section~\ref{sec:hybrid}).

\begin{figure*}[t!]
\centering
\includegraphics[width=.8\textwidth]{./Figures/TACAN_arch_v2}
%\vspace{-0.6cm}
\caption{Illustration of the architecture and the transmitter authentication protocol of TACAN. A master key is shared and a session key counter is synchronized between each ECU and the MN. The ECU and the MN generate the same session key from the master key and the session key counter, and they use it to generate and verify authentication messages, respectively. Unsuccessful reception and verification of authentication messages implies a possible CAN bus anomaly. 
The master key, the session key counter, and the generated session keys are stored securely in the TPM of the ECU and the MN.
}
\label{fig:TACAN_arch}
\end{figure*}

\subsection{TACAN architecture}
\label{sec:tacan_architecture}
As illustrated in Fig.~\ref{fig:TACAN_arch}, TACAN consists of in-vehicle ECUs and a centralized, trusted Monitor Node (MN).
The MN is installed by the manufacturer during production and requires direct physical access by authorized parties (e.g., an authorized repairs shop) to prevent potential tampering and compromises.
The deployed covert channels are configured during production or re-configured during maintenance to ensure successful establishment of one-way communication of authentication information from ECUs to the MN.

Similar to~\cite{hazem2012lcap,radu2016leia,herrewege2011canauth}, we assume that a master key (MK) is pre-shared between each ECU and the MN, and it is stored in the TPM. 
Updating of MKs (e.g., when adding or replacing an ECU) should again require direct physical access by authorized parties to the involved ECUs.
The procedure of key updating is outside the scope of this paper.
During operation, the ECU and the MN will generate the same session key (SK) from the MK and the synchronized SK  counter, and further use it to generate and verify authentication messages, respectively.
We now describe the transmitter authentication protocol in more detail.

% \begin{figure}[h!]
% \centering
% \includegraphics[width=1\columnwidth]{./Figures/protocol}
% \caption{Illustration of transmitter authentication protocol. \shaun{(Shaun: Radha asked me to make such a figure in the slides. Do we want a figure like this in the paper?) \giuseppe{probably good to have a similar figure also for the journal version. the periodic counter sync is referring to the actual global counter?}}
% }
% \label{fig:TACAN_arch}
% \end{figure}

\subsection{Transmitter Authentication Protocol}
\label{sec:transmission_authentication_protocol}
Inspired by the work in~\cite{radu2016leia}, the MN in TACAN performs unidirectional authentication of ECUs.
In this section, we summarize the key protocol parameters and describe the procedures of session key generation as well as authentication message generation and verification. 

\vspace{0.1cm}
\noindent \textbf{Authentication protocol parameters.} 
In TACAN, both the ECU that transmits CAN messages with ID or priority equal to $k$ \footnote{In our earlier work \cite{ying2019tacan}, we assumed one message ID per ECU. In practice, however, an ECU may transmit CAN messages with different IDs. In this case, TACAN needs to be deployed for each message ID. } and the MN store a tuple $\langle MK^{(k)}, C_s^{(k)}, SK^{(k)}, C_m^{(k)} \rangle$, where
\begin{itemize}
    \item The master key $MK^{(k)}$ is a long term pre-shared key that is used to generate the session key; 
    
    \item The session key counter $C_s^{(k)}$ is a counter that is incremented by one at every vehicle start-up or when $C_m^{(k)}$ overflows; it is used to generate the session key;
    
    \item The session key $SK^{(k)}$ is a key used to generate authentication messages for CAN messages with ID=$k$;
    
    \item The authentication message counter $C_m^{(k)}$ is a counter that is incremented by one before being used to generate the next authentication message. %, so as to provide freshness.
\end{itemize}
We assume that $MK^{(k)}$, $SK^{(k)}$ and $C_{s}^{(k)}$ are securely stored in the TPMs of both the ECU and the MN. 
 

% The parameters used by TACAN for the $n$ ECUs are summarized as follows:
% \begin{itemize}
%     \item The master key $MK^{(k)}$ with $k \in \{1,...,n\}$ is a pre-shared key between ECU $k$ and the MN.
    
%     \item The session key $SK^{(k)}$ with $k \in \{1,...,n\}$ is used to generate authentication messages for ECU $k$.
%     %used to generate the Message Authentication Code (MAC) or digest for transmitter authentication purposes.
    
%     \item The \shaun{authentication message counter} $C_{m}^{(k)}$ with $k \in \{1,...,n\}$ is an incremental value that stores the number of transmitted authentication messages for ECU $k$. 
%     This value is contained in the authentication message.
    
%     \item The \shaun{session key counter} $C_s^{(k)}$ with $k \in \{1,...,n\}$ represents a value updated on specific circumstances (e.g., car ignition, $C_m^{(k)}$ overflow) and it is used to generate $SK^{(k)}$. 
    
% \end{itemize}

% \giuseppe{Comment here on  what  parameters  (timing,  authenticationrelated)  need  to  be  pre-configured  between  ECUs  and  theMN.
% Also better to create another noindent with all the parameters description and, see above}

\vspace{0.1cm}
\noindent \textbf{Session key generation.}
The session key generation function takes a master key $MK^{(k)}$ and a session key counter $C_s^{(k)}$ as input and outputs a session key $SK^{(k)}$ (Fig.~\ref{fig:session_key_gen}).

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\columnwidth]{./Figures/session_key_gen}
    \caption{Session key generation for the ECU that transmits CAN messages with ID=$k$ and the MN. }
    \label{fig:session_key_gen}
\end{figure}

As we can see, both the ECU and the MN first increment $C_s^{(k)}$ by one, i.e., $C_s^{(k)} \leftarrow C_s^{(k)}+1$. 
Then, they perform the following operation on $C_s^{(k)}$ using $MK^{(k)}$,
\begin{equation}
    SK^{(k)} = HMAC(MK^{(k)},C_s^{(k)}),\nonumber
\end{equation}
where $HMAC(\cdot)$ refers to the Hash-based Message Authentication Code (MAC) algorithm \cite{krawczyk1997hmac}.
Implementations of the protocol are free to use whichever hashing algorithm for HMAC and sizes of keys that are deemed strong enough.
One possible choice would be HMAC-SHA256 and 256 bits for keys. 
%A suitable hashing algorithm for HMAC (e.g., HMAC-SHA256) as along with key lengths should be chosen carefully to meet the desired security requirements.
When a new session key is generated, $C_s^{(k)}$ is reset to zero. 

%Every time $SK^{(k)}$ is updated, $C_m^{(k)}$ will be reset to zero. On the MN side, the MN uses the same $MK^{(k)}$ and $C_s^{(k)}$ to compute $SK^{(k)}$.
%Counter synchronization is performed when $C_s^{(k)}$ is incremented. 
In the case of de-synchronized session key counters, a re-synchronization procedure such as the one in \cite{radu2016leia} will be needed, which may require message exchange between the ECU and the MN. 
The detailed design of such procedure is beyond the scope of this work. 

\vspace{0.1cm}
\noindent \textbf{Authentication message generation.}
As shown in Fig.~\ref{fig:auth_msg_gen}, the ECU that uses message ID $k$ increments $C_m^{(k)}$ by one and then generates the authentication message $A_m^{(k)}$ as follows: 
\begin{equation}
    A_{m}^{(k)} = C_m^{(k)} || HMAC(SK^{(k)}, C_m^{(k)}), \label{eq:A_m_structure} 
\end{equation}
where ``$||$'' denotes the concatenation of the counter value and the digest.
For the scope of this work, we assume that keys, counter values, and digests for TACAN are represented as bit strings. 

The generated authentication message is then transmitted using the covert channel and received by the MN.
Next, we will describe the verification procedure that happen on the MN side.

% \LinesNumbered
% \begin{algorithm}[h!]
% 	\SetKwInOut{Input}{Input}
% 	\SetKwInOut{Output}{Output}
% 	\Input{$SK^{(k)}$, $C_m^{(k)}$}
% 	\Output{$A_m^{(k)}$}
	
% 	$C_m^{(k)} \leftarrow C_m^{(k)} + 1$\;
% 	$A_m^{(k)} \leftarrow C_m^{(k)} || HMAC(SK^{(k)}, C_m^{(k)})$\;

% 	\textbf{return} $A_m^{(k)}$\;
% \caption{Authentication message generation}
% \label{pseudo:auth_msg_gen}
% \end{algorithm}
% \setlength{\textfloatsep}{3pt}

\begin{figure}[h!]
    \centering
    \includegraphics[width=.7\columnwidth]{./Figures/auth_msg_gen.pdf}
    \caption{Illustration of authentication message generation. }
    \label{fig:auth_msg_gen}
\end{figure}


\vspace{0.1cm}
\noindent \textbf{Authentication message verification.} 
Algorithm~\ref{pseudo:auth_msg_ver} describes the authentication message verification procedure. 
For each received authentication message $\hat{A}_m^{(k)}$, the MN first extracts the counter value $\hat{C}_m^{(k)}$ and the corresponding digest $\hat{h}$ (Line~\ref{algo:ver:line1}). 
Then the MN increments its authentication message counter $C_m^{(k)}$ by one and compares it against $\hat{C}_m^{(k)}$ (Lines \ref{algo:ver:line2}-\ref{algo:ver:line3}). 
If the counter values are the same, the MN computes the expected digest $h$ (Line~\ref{algo:ver:compute_mac}) and compares it against $\hat{h}$ (Line~\ref{algo:ver:compare_mac}). 
If the digests are the same, the algorithm returns True, which indicates successful authentication message verification.
On the other hand, the mismatch of either the counter values or the digests means verification failure and indicates a possible CAN bus anomaly. 

\LinesNumbered
\begin{algorithm}[h!]
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{$\hat{A}_m^{(k)}$, $SK^{(k)}$, $C_m^{(k)}$}
	\Output{True or False}
	
	$\hat{C}_m^{(k)}, \hat{h} \leftarrow \hat{A}_m^{(k)}$\; \label{algo:ver:line1}
	$C_m^{(k)} \leftarrow C_m^{(k)} + 1$\;\label{algo:ver:line2}
	\If{$\hat{C}_m^{(k)} = C_m^{(k)}$ \label{algo:ver:line3}}
	{
	    $h \leftarrow HMAC(SK^{(k)}, C_m^{(k)})$\;\label{algo:ver:compute_mac}
	    \If{ $\hat{h} = h$ \label{algo:ver:compare_mac}}
	    {
	       \textbf{return} True\;  
	    }\Else{
	        \textbf{return} False\;  
	    }
	}\Else 
	{
	    \textbf{return} False\; 
	}
\caption{Authentication message verification}
\label{pseudo:auth_msg_ver}
\end{algorithm}
\setlength{\textfloatsep}{3pt}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=.95\columnwidth]{./Figures/auth_msg_ver}
%     \caption{Authentication message verification for ECU $k$. }
%     \label{fig:session_key_ver}
% \end{figure}

\vspace{0.1cm}
\noindent \textbf{Authentication frame structure.}
In TACAN, authentication messages are independent of CAN messages. 
They are encapsulated in authentication frames and transmitted through the covert channel.
Each authentication frame consists of four fields:
1) a SOF field, 2) a Data field, 3) a CRC field, and 4) EOF field. 
The SOF and EOF fields indicate the start and the end of an authentication frame, and the CRC field is used for error detection and ensures data integrity.

Inspired by the CAN frame structure (Fig.~\ref{fig:can_frame_structure}), we use a single bit 0 for the SOF and a bit string of 7 consecutive 1's for the EOF. 
We use an 8-bit CRC (CRC-8), which is also part of the AUTOSAR specifications \cite{autosar2017crc}, but more bits may be needed if necessary. 
Compared to the CAN frame, there are no arbitration, control, or ACK fields in the authentication frame, as they are no longer needed. 
When there are no authentication bits that need to be transmitted, bits of value one will be transmitted to fill the gap between frames. 

In order to avoid confusion due to possible appearances of the EOF in the frame, the bit stuffing technique will also be used, which inserts one bit of opposite polarity after five consecutive bits of the same polarity (including the preceding stuffed bit). 
The stuffed frame can then be destuffed by the receiver.
Note that the same bit stuffing technique is also used in the CAN protocol to maintain bit-level timing synchronization.


% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=.8\columnwidth]{./Figures/auth_frame_structure_v3}
%     \caption{Illustration of the authentication frame structure. 
%     %Each authentication frame consists of a SOF field, an authentication message (the payload), and the EOF field. 
%     }
%     \label{fig:auth_frame_structure}
% \end{figure}

As shown in Eq.~(\ref{eq:A_m_structure}), each authentication message contains a counter value and its digest.
A 24-bit counter can already last for 46+ hours for 10-ms CAN messages before having an overflow even in per-message authentication. 
While we assume a 24-bit counter in this work, fewer bits may be used in practice due to two reasons.
First, authentication messages in TACAN are transmitted in a much lower frequency, which means that the counter overflow will take a much longer time.
Second, since it is a monotonic counter incremented by one for every frame, the transmitter may only transmit the last few bits of the counter value to keep the receiver synchronized in the case of occasionally corrupted frames. 

As for the digest, instead of transmitting the entire digest that are usually hundreds of bits long, the transmitter may truncate each digest to several bits to reduce the transmission time (e.g., using the least significant 8 bits or XORing all bytes together to create a condensed 8-bit version of the digest, as in~\cite{kurachi2014cacan,szilagy2008flexible}).
In practice, the number of bits in the shortened version should be chosen appropriately to achieve a desirable security level.
%If we choose an 8-bit digest, then each $A_m$ is 32 bits, but the length of $A_m$ that is actually transmitted may exceed 32 bits due to bit stuffing. 


==> TACAN Extension (arXiv)/Sections/tacan_hybrid.tex <==
\subsection{Hybrid Covert Channel}
\label{sec:hybrid}
Since the IAT-based and LSB-based covert channels are orthogonal to each other, it leads to a natural question whether the two covert channels can be combined to construct a hybrid channel to achieve a larger throughput. 
In this hybrid covert channel, the transmitter will split the authentication message into two parts and transmit them through the two covert channels separately. 
Then the receiver will receive and reassemble the two parts into one piece.
In this work, we are interested in answering the following question: how to choose the splitting ratio $\alpha$ ($0\leq\alpha\leq 1$) such that the two parts will be transmitted roughly over the same duration. 

% \vspace{0.1cm}
% \noindent \textbf{Choosing the Splitting Ratio.}
Given $N_m$ bits for the authentication message and $N_o$ bits for other fields (SOF, CRC, and EOF), if we ignore bit stuffing, then there are a total of $\lceil\alpha N_m \rceil + N_o$ bits and $\lceil(1-\alpha) N_m \rceil + N_o$ bits transmitted over the IAT-based and LSB-based covert channels, respectively.

If the IAT-based covert channel is using a window length of $L_{1}$ and the LSB-based covert channel is using $L_2$ LSBs, then requiring the same transmission duration means
\begin{equation*}
    (\lceil\alpha N_m \rceil + N_o)L_1 = (\lceil(1-\alpha) N_m \rceil + N_o) /L_2.
\end{equation*}
Ignoring the ceiling function, we have \begin{equation}
    \alpha = \frac{N_m + N_o(1 - L_1 L_2)}{N_m(1+L_1 L_2)} \times 100\%. \label{eq:splitting_ratio}
\end{equation}
While $\alpha$ computed in in Eq.~(\ref{eq:splitting_ratio}) is not the optimal value $\alpha^*$ that leads to two partitions of equal length after bit stuffing, it will be close to $\alpha^*$, which provides a reasonable starting point for further iteration.
Note that $\alpha$ is less than or equal to $0$, it means that only the LSB-based covert channel should be used.
%\rev{In Section~\ref{sec:eval:throughput}, we will discuss the throughput gain in more detail.}

As an example, suppose $N_m=32$, $N_o=16$, $L_1=1$ and $L_2=1$. 
In this case, the two covert channels have similar throughput and we have $\alpha = 50.0\%$.
Nevertheless, if $L_1$ is increased from $1$ to $2$,  $\alpha$ quickly drops to $16.7\%$.
With $L_1=3$, $\alpha$ becomes $0$, which means that it is not advantageous to deploy the hybrid covert channel.


==> TACAN Extension (arXiv)/Sections/tacan_iat_based.tex <==
\subsection{IAT-Based Covert Channel}
\label{sec:IAT_based_covert_channel}
Fig.~\ref{fig:timing_based_covert_channel} illustrates the IAT-based covert channel for periodic CAN messages. 
In this covert channel, the ECU embeds the authentication bits into the ITTs of CAN messages, which can be extracted from the IATs by the MN. 
By verifying the received authentication message, the MN can authenticate the transmitter.

In the rest of this section, we will first motivate the design of the IAT-based covert channel through observations, and then present the modulation/demodulation schemes. 
After that, we will discuss the impact of two key parameters, that is, the window length $L$ and the added deviation $\delta$ on the bit error probability and the CAN bus schedulability.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth]{./Figures/timing_based_covert_channel.pdf}
    \caption{Illustration of the IAT-based covert channel. Each ECU embeds its authentication message $A_m$ into the ITTs of CAN messages, which can be observed and extracted by the MN through IATs. By verifying the received authentication message $\hat{A}_m$, the MN can verify the authenticity of the ECU. }
    \label{fig:timing_based_covert_channel}
    %\vspace{-0.3cm}
\end{figure}

\vspace{0.1cm}
\noindent \textbf{Observations.}
From Eq.~(\ref{eq:inter_arrival_time}), we observe that if an amount of deviation $\delta$ is added to (or subtracted from) the ITTs, the receiver will see a corresponding change in the IATs.
Hence, one simple scheme is to set $\Delta t_i=T+\delta$ for transmitting a bit $0$ and $\Delta t_i=T-\delta$ for transmitting a bit $1$.

Taking message 0x020 from the 2010 Toyota Camry \cite{toyota2010dataset} as an example, we plot its IAT distributions with added deviations in Fig.~\ref{fig:example_iat_distribution_L-1}, where $T=10$ ms and $\delta = 0.01T = 0.1$ ms. 
While adding a small deviation $\delta$ does lead to a shift in the IAT distribution, the two distributions are still overlapping with each other, indicating possible bit errors due to the noise caused by the CAN traffic. 

In order to reduce bit errors, one way is to average the IATs with a window length of $L$ at the receiver to smooth out the noise.
As we can see in Fig.~\ref{fig:example_iat_distribution_L-4}, 
%the clusters are completely separated from each other after performing running average.
performing running averages can effectively separate the two clusters from each other.
To support the computation of running averages at the receiver, the transmitter needs to transmit the same bit over $L$ consecutive ITTs. 
The above observations motivate the design of the IAT-based covert channel.

Note that when the probability of bit errors is reasonably small, one may also consider Error Correction Coding (ECC) techniques that are widely used in communications \cite{goldsmith2005wireless} to detect and recover occasional bit errors. 
Nevertheless, the use of ECC techniques will complicate the design of covert channels and introduce overheads.
As we will show later in Section~\ref{sec:evaluation}, since the probability of consecutive corrupted authentication frames is small, it is acceptable to not recover the bit errors in a particular frame.


\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[trim=0cm 0.3cm 0cm 0cm,clip=true,width=\textwidth]{Figures/example_iat_distribution_L-1.pdf}
        \caption{}
        \label{fig:example_iat_distribution_L-1}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.48\columnwidth}
        \includegraphics[trim=0cm 0.3cm 0cm 0cm,clip=true,width=\textwidth]{Figures/example_iat_distribution_L-4.pdf}
        \caption{}
        \label{fig:example_iat_distribution_L-4}
    \end{subfigure}
    %\vspace{-0.2cm}
    \caption{Example of IAT distributions of message 0x020 from the Toyota dataset at the receiver side (a) without running average ($L=1$) and (b) with running average ($L=4$).} 
    \label{fig:example_iat_distribution}
    %\vspace{-0.2cm}
\end{figure}

\vspace{0.1cm}
\noindent \textbf{Modulation.} 
The transmitter uses the following modulation scheme to embed a bit into the ITTs of CAN messages,
\begin{equation*}
    \Delta t_j =
    \begin{cases}
        T + \delta, & \text{ if } b_i = 0\\
        T - \delta, & \text{ if } b_i = 1
    \end{cases},
\end{equation*}
where $j \in [iL, (i+1)L)$. 
This is essentially the Binary Phase Shift Keying (BPSK) modulation in the communication theory \cite{goldsmith2005wireless}.
While more than two levels may be used to increase the throughput, we consider only two levels in this work to minimize the impact on the CAN bus schedulability.

\vspace{0.1cm}
\noindent \textbf{Demodulation.} 
From Eq.~(\ref{eq:inter_arrival_time}), we know that the original IATs are $\Delta a_j = T/(1+S) + n_j$. 
When $\Delta t_j$ is changed to $T \pm \delta$, the receiver will observe
\begin{equation*}
    \Delta a_j =\frac{T + (2 b_i - 1) \delta}{1+S} + n_j,
\end{equation*}
where $b_i \in \{0, 1\}$ is the transmitted bit and $j \in [iL, (i+1)L)$.
In this work, we assume that $\eta_j$'s are i.i.d. Gaussian random variables, i.e., $\eta_j \sim N(d, \sigma_\eta^2)$.
Hence, we have $n_j=\eta_j-\eta_{j-1} ~\sim N(0, \sigma^2)$, where $\sigma^2=2\sigma_\eta^2$.

In order to demodulate the authentication message from the IATs, the MN needs to perform three steps: 1) computing running averages, 2) sampling, and 3) thresholding. 
In the first step, the MN computes the running averages of window length $L$ as below,
\begin{align}
    \Delta \bar{a}[i] &= \frac{1}{L} \sum_{j=0}^{L-1}\Delta a_{i+j} \nonumber \\
    &= \frac{1}{1+S} \left( \frac{1}{L}  \sum_{j=0}^{L-1}\Delta t_{i+j} \right) + \frac{1}{L}(\eta_{i+L-1} - \eta_{i-1}). \label{eq:running_average}
\end{align}
From Eq.~(\ref{eq:running_average}), we can see that the noise term is reduced by a factor of $L$ and the resulting variance of IATs is $2\sigma_{\eta}^2/L^2$.

After computing the running averages $\{\Delta \bar{a}[i]\}$, the MN needs to sample every $L$ values with a correct sampling offset $\tau^*$ and obtains $\{\Delta \bar{a}[iL + \tau^*]\}$.
From the communication theory \cite{goldsmith2005wireless},
%(Section 5.1.4 in \cite{goldsmith2005wireless}), 
we know that the optimal receiver minimizes the bit error probability $P_e$ by selecting the output $\hat{b}[i]$ that maximizes $1-P_e=\text{Pr}(b_i \text{ sent } | \Delta \bar{a}[iL + \tau^*] \text{ received})$.
If we assume that bits 0 and 1 are transmitted with equal probabilities, then the maximum likelihood decision criterion is
\begin{equation*}
    \hat{b}[i] =
    \begin{cases}
        0, & \text{ if } \Delta \bar{a}[iL+\tau^*] \geq \Gamma,\\
        1,  & \text{ otherwise },
    \end{cases}
\end{equation*}
where $\Gamma=  \frac{T}{1+S}$ (Eq.~(\ref{eq:IAT_mean})), that is, the decision threshold is the mean of original IATs or the observed message period. 
Lastly, the MN can decode $A_m$ from the bit string $\{\hat{b}[i]\}$. 

Note that it is not necessary for the receiver to be synchronized with the transmitter for the sampling purposes, because the receiver can determine the correct sampling offset $\tau^*$ by itself as follows, 
\begin{equation}
    \tau^* = \arg \max_{\tau} \sum_i \left|\Delta \bar{a}[iL+\tau] - \Gamma \right|,
    \label{eq:optimal_tau}
\end{equation}
where $\tau\in \{0,1,..,L-1\}$.
That is, $\tau^*$ is the integer value that maximizes the total distance between each sample and the decision threshold. 

\vspace{0.1cm}
\noindent \textbf{Impact of $\delta$ and $L$ on bit error probability.}
From our previous discussion, we see that $L$ and $\delta$ are the two key parameters that affect the bit error performance of the IAT-based covert channel. 
In this section, we analytically model the bit error probability $P_e$ as a function of $L$ and $\delta$. 

First of all, based on our previous assumption of Gaussian noise, we have 
\begin{equation}
    \Delta \bar{a}[iL + \tau^*] ~\sim N\left( \frac{T + (2b_i-1)\delta }{1+S}, \frac{\sigma^2}{L^2} \right), \label{eq:distribution_of_sampled_IAT}
\end{equation}
where $b_i \in \{0,1\}$ and $\sigma^2 = 2\sigma^2_\eta$ (Eq.~(\ref{eq:noise_variance})).
Let $P_{e,0}$ and $P_{e,1}$ be the bit error probabilities conditioned on bits 0 and 1 being transmitted, respectively. 
Then we have
\begin{align*}
P_{e,0} &= \text{Pr}(\Delta \bar{a}[iL+\tau^*] < \Gamma | b_i = 0), \\
P_{e,1} &= \text{Pr}(\Delta \bar{a}[iL+\tau^*] \geq \Gamma | b_i = 1).
\end{align*}
According to Eq.~(\ref{eq:distribution_of_sampled_IAT}), we know that
\begin{align}
    P_{e,0} = \text{Pr}\left(Z < \frac{ -\delta/(1+S)}{\sigma/L}\right) = Q \left( \frac{L \delta}{(1+S)\sigma } \right) \nonumber,
\end{align}
where $Z\sim N(0,1)$ is the standard Gaussian random variable and $Q(x)\triangleq \frac{1}{\sqrt{2\pi}} \int_{z}^{\infty} exp(-\frac{z^2}{2}) dz$ is the Q function. 
Due to the symmetry, we have $P_{e,0}=P_{e,1}$. 

Assuming equally likely probabilities of bits 0 and 1, i.e., $P_0=P_1=0.5$, the total error bit probability is
\begin{equation}
    P_e = P_{e,0}\cdot P_0 + P_{e,1} \cdot P_1 =Q \left( \frac{L \delta}{(1+S)\sigma} \right). \label{eq:bit_error_probability}
\end{equation}

From Eq.~(\ref{eq:bit_error_probability}), we see that increasing $L$ and $\delta$ would have the same effect on $P_e$. 
%Fig.~\ref{fig:bit_error_probability} also plots $P_e$ as a function of $\delta/\sigma_n$ for different $L$ values, where the ratio  of $\delta$ and $\sigma_n$ captures the signal-to-noise relationship.
Nevertheless, increasing $L$ will reduce the covert channel throughput, whereas increasing $\delta$ could potentially affect the schedulability of the CAN bus, as we will explain in the next section.
Therefore, in the case of fixed $\delta$, it makes full sense to choose the smallest $L$ value, while keeping $P_e$ less than or equal to a given limit $\epsilon$. 
From Eq.~(\ref{eq:bit_error_probability}), we have
\begin{equation}
    L_{\min} = \left\lceil \frac{(1+S)\sigma}{\delta} Q^{-1}(\epsilon) \right\rceil,
\end{equation}
where $\lceil \cdot \rceil$ is the ceiling function.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=1\columnwidth]{./Figures/bit_error_probability.pdf}
%     \caption{Bit error probability ($P_e$) as a function of the ratio between the added deviation ($\delta$) and the standard deviation of IATs ($\sigma$) with different values of the window length ($L$). }
%     \label{fig:bit_error_probability}
%     %\vspace{-0.3cm}
% \end{figure}

% \new{
% \vspace{0.1cm}
% \noindent \textbf{Estimation of $L$:}
% On the receiver side, the MN can collect enough samples and estimate the value of $L$ as described in Algorithm~\ref{pseudo:estimating_L}. 

% }
% We now describe how the MN can estimate the window length $L$ and the sampling offset $\tau^*$. 

% \shaun{(Basic procedure: for $L$ from $1$ to $L_{\max}$, choose the $\tau^*$ that maximizes Eq.(\ref{eq:optimal_tau}). After thresholding, check if the maximum length of bits is equal to $N_m$ (the number of authentication bits).)}

% \shaun{(Assume timing parameters (e.g., $T$ and $\delta$) and authentication parameters (e.g., $N_f$) are pre-shared. Focus on estimation of $L$ and $\tau$)}
% We now describe how the MN can estimate covert channel parameters, namely, $L$, $\delta$, and $\tau^*$. 

% Let the sampling offset be $\tau$ and the $j$-th sample be $\Delta \bar{a}[jL+\tau]$. 
% If $\tau$ is correctly chosen, the total distance between each modulated sample and the reference level ($\kappa$) should be maximized, i.e.,
% \begin{equation}
%     \tau^* = \arg \max_\tau \sum_j \left|\Delta \bar{a}[jL+\tau] - \kappa \right|. 
%     \label{eq:optimal_tau}
% \end{equation}


% \LinesNumbered
% \begin{algorithm}[h!]
% 	\SetKwInOut{Input}{Input}
% 	\SetKwInOut{Output}{Output}
% 	\SetKw{KwBy}{by}
% 	\Input{$\{\Delta a\}$ (IATs), $N_m$ (number of bits in $A_m$), $\Gamma$ (decision threshold), $\gamma$ (a value between 0 and 1)}
% 	\Output{$L$ (window length)}
	
% 	$L \leftarrow 1$ \;
% 	\While{True}
% 	{
% 	    $\{\Delta \bar{a}\} \leftarrow$ {\tt running\_average} $(\{\Delta a\}, L)$\;
% 	    $\tau^* \leftarrow \arg \max_{0\leq \tau \leq L-1} \sum_j \left|\Delta \bar{a}[jL+\tau] - \kappa \right|$\;
% 	    $\{\hat{b}\} \leftarrow $ {\tt thresholding} $(\{\Delta \bar{a}\}, L, \tau^*)$\;
% 	    $segments \leftarrow$ {\tt split} $(\{\hat{b}\},~ ``\_")$\;
% 	    $Count \leftarrow 0$\;
% 	    \For{each $segment$ in $segments$}
% 	    {
% 	        \If{{\tt length}($segment$) $== N_m$}{$Count \leftarrow Count + 1$}
% 	    }
%         \If{$Count \geq \gamma \cdot$ {\tt length}$(segments)$ }
%         {
%             \textbf{break}\;
%         }\Else{$L \leftarrow L + 1$\;}
% 	}

% 	\textbf{return} $L, \tau^*$\;
% \caption{Window length estimation}
% \label{pseudo:estimating_L}
% \end{algorithm}
% \setlength{\textfloatsep}{3pt}

\vspace{0.1cm}
\noindent \textbf{Impact of $\delta$ on CAN bus schedulability:}
Timing on the CAN bus is closely related to its schedulability.
A CAN bus is schedulable if and only if all the messages on the bus are schedulable, and a message with ID $k$ is schedulable if and only if its worst-case response time (denoted as $R_k$) is less than or equal to its deadline (denoted as $D_k$). 

According to \cite{davis2007controller}, $R_k$ is defined as the longest time from the initiating event (that puts the message in the transmission queue) occurring to the message being received by the nodes that require it.
It consists of three parts: 1) the queuing jitter, 2) the queuing delay, and 3) the transmission time. 
The queuing delay further consists of the blocking delay (due to ongoing transmissions of lower priority messages) and the interference (due to the arbitration process when competing with higher priority messages).

Since the IAT-based covert channel introduces a deviation of $\delta$, its effect is equivalent to decreasing the message period (defined as the minimum inter-transmission time) and increasing the queuing jitter. 
By applying the schedulability analysis in \cite{davis2007controller}, we can show that the impact of $\delta$ on the worst-case response time
%on the CAN bus schedulability 
is threefold: 1) increase in the queuing jitter by a fixed amount ($\delta$), 2) increase in the blocking delay by a bounded amount of time, and 3) increase the message transmission time of higher priority messages by a certain percentage ($\delta/T$). 
Therefore, to achieve the effective use of the IAT-based covert channel, TACAN parameters (notably $\delta$) need to be experimentally obtained and fine tuned prior to deployment to ensure the schedulability of the CAN bus.
A detailed discussion is provided in Appendix A. 
%Appendix~\ref{appendix:schedulability}.


==> TACAN Extension (arXiv)/Sections/tacan_lsb_based.tex <==
\subsection{LSB-Based Covert Channel}
\label{sec:lsb_based}
In this section, we present the LSB-based covert channel, which %is a non-timing-based covert channel that
embeds the authentication messages inside the LSBs of the data payload of normal CAN messages transmitted by an ECU, as illustrated in Fig.~\ref{fig:lsb_scheme}.
Unlike the IAT-based covert channel, the LSB-based covert channel is also applicable to aperiodic CAN messages.
For the scope of this work, we use the CAN data frames to develop our methodology.

\vspace{0.1cm}
\noindent \textbf{Observations.}
In order to transmit authentication messages over the CAN bus, it is common to leverage the existing fields of a CAN message, such as the data field (at least one byte) and the extended ID field, or simply introduce additional CAN messages~\cite{kurachi2014cacan,hazem2012lcap,groza2012libra}.
In practice, however, there may not be any unused bytes in the CAN message or the CAN bus is already heavily loaded, which makes the above approaches difficult to deploy. 
In TACAN, the objective is to authenticate the transmitter instead of each CAN message, and thus authentication messages are transmitted much less frequently. 
% Hence, each CAN message only need to carry a few authentication bits (e.g., one or two bits).  
If we can spread the bits of an authentication message across multiple CAN messages, each of which carries only a few authentication bits (e.g., one or two bits), we can then alleviate the payload shortage and avoid traffic overheads.

On the other hand, we also observe that CAN messages are often used to convey sensor values, most of which are floating values represented in bits. 
Therefore, the $L$ LSBs (e.g., $L=1$ or $2$) of each such CAN message may be used for transmitting authentication bits without causing significant degradation in accuracy. 

Taking the 2010 Toyota Camry \cite{toyota2010dataset} as an example, there are at least $7$ messages out of $42$ that carry sensor values (e.g., wheel speeds, engine speed, vehicle speed, odometer, brake pressure, steering angle) \cite{toyota2010dataset}. 
We would expect more CAN messages that carry sensor values in newer automobiles.
The above observations motivate our design of LSB-based covert channels.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{./Figures/lsb_scheme.pdf}
    \caption{Illustration of LSB-based covert channel. The transmitting ECU embeds the authentication message into the LSBs of multiple normal CAN messages (with the same ID), which can be extracted and verified by the Monitor Node.}
    \label{fig:lsb_scheme}
    % \vspace{-0.3cm}
\end{figure}

\vspace{0.1cm}
\noindent \textbf{Embedding $A_m$ to LSBs.} 
The embedding procedure is considered as a sub-layer between the Application and the Data Link layers. 
The basic idea is as follows: for each message $A_m$, the transmitter substitutes the least significant $L$ bits of the CAN message with the next $L$ bits in $A_m$. 
No modification is needed if the $L$ bits happen to be the same.

As provided in Algorithm \ref{pseudo:ecu_tx}, an authentication frame $A_f$ is first constructed from $A_m$  (Line~\ref{algo:lsb:A_f}). 
%Since the authentication frames are generated and transmitted continuously, the SOF of the next authentication frame indicates the end of the previous one.
When the new data field content $d_{field}$ is received from the upper (Application) layer, the least significant $L$ bits of the selected byte $\beta$ in $d_{field}$, denoted as $bin(d_{field}(\beta))_L$, are compared with the next $L$ bits of $A_f$: if the bits of interest are different, then the substitution occurs; otherwise, $d_{field}$ is not modified (Lines~\ref{algo:lsb:line3}-\ref{algo:lsb:line7}).
The same process is repeated for each new authentication message. 

% \begin{table}[h]
% % 	\footnotesize
% 	\centering
% 	\caption{Notation of LSB-based covert channel algorithms.}
% 	\begin{tabular}{|c|l|}
% 		\hline
% 		\textbf{Notation} & \textbf{Description} \\
% 		\hline
% 	%	$A_s$  & Start of Frame (SOF) \\ \hline
% 		$A_m$ & Authentication message \\ \hline
% 		$A_f$ & Authentication frame \\ \hline
% 		$d_{field}(\cdot)$ & Data field of CAN data frame \\ \hline
% 		$\beta$ & Selected bytes (value) \\ \hline
% 		$bin(\cdot)_L$ & Least significant $L$ bits \\ \hline
% 	\end{tabular}
% 	\label{table:LSB_notation}
% 	\normalsize
% \end{table}

\LinesNumbered
\begin{algorithm}[h!]
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
% 	\Input{$A_m$, $L$}
	%\Input{$A_s$, $L$, $\{d_{frame}\}$ (data frames to be transmitted)}
	%\Output{$\{d_{frame}\}$ (modified data frames)}
	%$A_f \leftarrow A_s||A_m$ (with bit stuffing)\; 
	Construct $A_f$ from $A_m$ (with bit stuffing)\;
	\label{algo:lsb:A_f}
	$i \leftarrow 0$\; 
	\While{$i < length(A_f)$ \label{algo:lsb:line3}} 
	{
	    Receive $d_{field}$ from the upper (Application) layer\;
	    \If{$bin(d_{field}(\beta))_L \neq A_f[i:i+L-1]$}
		{
		    $bin(d_{field}(\beta))_L = A_f[i:i+L-1]$\;
		}
        $d_{frame} \leftarrow d_{field}(\gamma)$\;
		$i \leftarrow i + L$\; \label{algo:lsb:line7}
		Send $d_{field}$ to the lower (Data Link) layer\;
	}

	\textbf{return}\;
\caption{Embedding $A_m$ to LSBs}
\label{pseudo:ecu_tx}
\end{algorithm}
\setlength{\textfloatsep}{3pt}

\vspace{0.1cm}
\noindent \textbf{Extracting $A_m$ from LSBs.} 
On the receiver side, the MN extracts the $L$ LSBs from every received CAN message and reconstructs the authentication message.
If the MN fails to verify the authentication message, it will raise an alert that indicates possible compromise of the transmitting ECU or malicious exploitation of the CAN bus.

The extracting procedure is described in Algorithm \ref{pseudo:mon_rx}. 
Once the MN detects the SOF flag, it will start extracting the $L$ LSBs from the designated byte $d_{field}(\beta)$ and appending them to $\hat{A}_f$ (Lines~\ref{algo:lsb:extract:line1}-\ref{algo:lsb:extract:line5}). 
When the EOF flag is detected in $\hat{A}_f$, the MN will perform bit destuffing on $\hat{A}_f$ and extract the authentication message $\hat{A}_m$ (Line~\ref{algo:lsb:extract:line6}). 
Then it will listen for the SOF of the next incoming frame. 

\LinesNumbered
\begin{algorithm}[h!]
	\SetKwInOut{Input}{Input}
	%\SetKwInOut{Output}{Output}
	%\Input{$d_{field}, L$}
% 	\Input{$L$}
	%\Output{$d_{frame}$}
	
	\If{SOF is detected\label{algo:lsb:extract:line1}} 
	{
	    Initialize $\hat{A}_f$ to an empty bit string\;
	    \While{EOF is not detected in $\hat{A}_f$}{
	        Receive $d_{field}$ from the Data Layer layer\;
	        Append $bin(d_{field}(\beta))_L$ to $\hat{A}_f$\; \label{algo:lsb:extract:line5}
	    }
	    Destuff $\hat{A}_f$ and extract $\hat{A}_m$\;  \label{algo:lsb:extract:line6}
	}
	
	\textbf{return} $\hat{A}_m$\;
	
	\caption{Extracting $A_m$ from LSBs}
	\label{pseudo:mon_rx}
\end{algorithm}
\setlength{\textfloatsep}{5pt}

==> TACAN Extension (arXiv)/Sections/tacan_offset_based.tex <==
\subsection{Offset-Based Covert Channel}
\label{sec:offset_based}
The idea of the offset-based covert channel is very similar to the IAT-based covert channel (Figure~\ref{fig:timing_based_scheme}).
The main difference is that the former performs running average on IATs (including the added deviations) to smooth out the noise, while the later aims to accumulate the deviations to differentiate the modulated samples from noise. 
Our observations about clock offsets are as follows. 

\vspace{0.1cm}
\noindent \textbf{Observations.}
According to our timing model in Section~\ref{sec:system_model} and Eq.~(\ref{eq:arrival_timestamp}), we have $t_i=\sum_{j=1}^i \Delta t_j$, $a_0=\eta_0$, and $a_i=t_i/(1+S)+\eta_i$. 
Since the receiver only knows the nominal period ($T$) of the targeted message, it computes the observed clock offset as the difference between the expected elapsed time (up to message $i$) at the transmitter and the actual elapsed time at the receiver, i.e.,
\begin{equation}
    \hat{O}_i = iT - (a_i - a_0) = iT - \frac{1}{1+S} \sum_{j=1}^i \Delta t_j + \eta_0 - \eta_i. \nonumber
\end{equation}
As we can see, if the transmitter adds $\delta$ to $L$ consecutive ITTs ($\Delta t_j = T+\delta$ for $j=1,...,L$), the deviations will accumulate and lead to a decrease of $\delta L/(1+S)$ in $\hat{O}_i$.
Hence, by monitoring the changes in $\hat{O}_i$, the receiver can determine the transmitted bits and extract $A_m$ from clock offsets. 
The above observations motivate our design of offset-based covert channels. 

% On CAN buses with heavy traffic, the noise in ITTs caused byarbitration can be very significant, and it would require a largeδvalue in order to establish a reliable ITT-based covert channel.Taking the message with ID=0x0C5 andT=10ms in the EcoCAR[1] as an example

% \begin{figure}[ht!]
%     \centering
%     \begin{subfigure}[b]{0.48\columnwidth}
%         \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_offset_based_CC_0c5_IATs}
%         \caption{}
%         \label{fig:example_offset_based_CC_0c5_IATs}
%     \end{subfigure}
%     ~
%     \begin{subfigure}[b]{0.48\columnwidth}
%         \includegraphics[trim=0cm 0cm 1.3cm 1.3cm,clip=true,width=\textwidth]{Figures/example_offset_based_CC_0c5_offsets}
%         \caption{}
%         \label{fig:example_offset_based_CC_0c5_offsets}
%     \end{subfigure}
%     \caption{Example message with ID=0x0C5 and a period of $T=10$ ms from the EcoCAR \cite{ecocar}. (a) The IATs vary between $9.3$ ms and $10.7$ ms. (b) Accumulated offsets. }
%     \label{fig:example_offset_based_CC_0c5}
% \end{figure}

\vspace{0.1cm}
\noindent \textbf{Embedding $A_m$ into ITTs.}
Different from the IAT-based covert channel (Section~\ref{sec:IAT_based_covert_channel}), the transmitter embeds each bit of $A_f$ into $L$ consecutive ITTs as follows,
\begin{equation*}
    \Delta t_j =
    \begin{cases}
        T - \delta, & \text{ if } b_i = 0,\\
        T + \delta, & \text{ if } b_i = 1,\\
        T, & \text{ else},
    \end{cases}
\end{equation*}
\rev{for $j \in [iL, (i+1)L),$} and 
\begin{equation*}
    \Delta t_j =
    \begin{cases}
        T + \delta, & \text{ if } b_i = 0,\\
        T - \delta, & \text{ if } b_i = 1,\\
        T, & \text{ else},
    \end{cases}
\end{equation*}
\rev{for $j \in [iL+L/2, (i+1)L)$}, where $L$ is assumed to be an even integer. 
In other words, in order to transmit a bit 0/1, the transmitter adds $-\delta$/$\delta$ to the first $L/2$ ITTs and then subtracts $-\delta$/$\delta$ from the following $L/2$ ITTs so that the observed clock offset returns to the reference level after the transmission of each bit.

\vspace{0.1cm}
\noindent \textbf{Extracting $A_m$ from Offsets.}
On the receiver side, the monitor node records the arrival timestamps and processes the IATs in batches. 
Since each $A_f$ has $n_f$ bits and each bit is modulated into $L$ consecutive ITTs, a total number of $N = n_f L$ consecutive IATs belong to the same $A_f$, where $N$ is referred to as the batch size. 

Denote the $i$-th IAT in the $k$-batch as $\Delta a_{k,i}$, where $1 \leq i \leq N$.  
Then the observed clock offset with respect to the beginning of the current batch up to the $i$-th IAT is 
\begin{equation*}
    \hat{O}_{k}[i] = iT - \sum_{j=1}^{i} \Delta a_{k,j}.
\end{equation*}
Let $\kappa = (\max(\hat{O}_{k}[i]) + \min(\hat{O}_{k}[i]))/2$ be the midpoint (assuming that at least a bit 0 and a bit 1 are transmitted), which is considered as the reference level of clock offsets.
\rev{Since clock skew is usually very small (100s of ppm) and we are computing batch-wise clock offsets, the impact of clock skew is small, and thus we assume that the $\kappa$ is constant for the duration of a batch\footnote{In the case of very large clock skew (e.g., 1000s of ppm), there will be a linear trend due to clock skew in batch-wise clock offsets and thus the reference level may not be constant. We leave the detrending process of clock offsets as future work.}.}
%, which is considered as the reference level of clock offsets\footnote{Note that since clock skew is usually very small (100s of ppm) and we are computing batch-wise clock offsets, the impact of clock skew is small. Hence, we assume that the (possibly non-zero) reference level is constant for the duration of a batch. Nevertheless, in the case of very large clock skew (e.g., 1000s of ppm), there will be a linear trend due to clock skew in batch-wise clock offsets and thus the reference level may not be constant. We leave the detrending process of clock offsets as future work.}. 
Since each bit affects $L$ IATs, the receiver needs to sample $\{\hat{O}_{k}[i]\}$ every $L$ values with a sampling offset of $\tau$ and obtain the $j$-th sample as $\hat{O}_{k}[jL + \tau]$. 
If $\tau$ is correctly chosen, then the total distance between each sample and the reference level should be maximized, i.e.,
\begin{equation*}
    \tau^* = \arg \max_{\tau} \sum_j | \hat{O}_{k}[jL + \tau] - \kappa|. 
\end{equation*}
Then the receiver converts the sampled values to bits through the following threhsolding-based scheme,
\begin{equation*}
    \hat{b}_j =
    \begin{cases}
        0, & \text{ if } \hat{O}_{k}[jL + \tau^*] > \Gamma_u,\\
        1,  & \text{ if } \hat{O}_{k}[jL + \tau^*] < \Gamma_l,\\
        \text{{\tt \_}}, & \text{ else, }%   // (Silence bit)}
    \end{cases}
\end{equation*}
where $\Gamma_l=\kappa - \frac{1}{4}\delta L$ and $\Gamma_u=\kappa + \frac{1}{4}\delta L$ are the lower and upper thresholds, respectively\rev{, and ``\_'' is the silence bit}. 
The term of $\frac{1}{4}\delta L$ is due to the fact that $\delta$ is added to (or subtracted from) $L/2$ consecutive ITTs, and thus the maximum total deviation is $\pm \frac{1}{2} \delta L$. 
The midpoints between $\kappa$ and $\kappa \pm \frac{1}{2} \delta L$ are chosen as thresholds. 
Eventually, $A_m$ is extracted by concatenating all decoded bits and splitting them at the silence bits. 

\vspace{0.1cm}
\noindent \textbf{Impact on CAN bus schedulability.} As we have shown, in both the IAT-based and offset-based covert channels, a certain amount of deviation is added to the ITTs.
As a result, it may increase the worst-case response time of CAN messages, which is defined as the longest time from the initiating event (that puts the message in the transmission queue) occurring to the message being received by the nodes that require it.
If we apply the schedulability analysis in \cite{davis2007controller} to TACAN, we can show that the effect of TACAN is equivalent to increasing the blocking delay by a constant amount of time (hundreds of $\mu$s) and increasing the message transmission time by a small percentage. 
Therefore, to achieve effective use of covert channels, TACAN parameters need to be experimentally obtained and fine tuned prior to deployment to ensure the schedulability of the CAN bus.
%to ensure the schedulability of the CAN bus.
A more detailed discussion is provided in Appendix~\ref{appendix:schedulability}.


\new{Generalize this approach to messages with large clock skew}
